A Model-Based Approach to Anomaly Detection Trading Detection Time and False Alarm Rate

The complexity and ubiquity of modern computing systems is a fertile ground for anomalies, including security and privacy breaches. In this paper, we propose a new methodology that addresses the practical challenges to implement anomaly detection approaches. Specifically, it is challenging to define normal behavior comprehensively and to acquire data on anomalies in diverse cloud environments. To tackle those challenges, we focus on anomaly detection approaches based on system performance signatures. In particular, performance signatures have the potential of detecting zero-day attacks, as those approaches are based on detecting performance deviations and do not require detailed knowledge of attack history. The proposed methodology leverages an analytical performance model and experimentation and allows to control the rate of false positives in a principled manner. The methodology is evaluated using the TPCx-V workload, which was profiled during a set of executions using resource exhaustion anomalies that emulate the effects of anomalies affecting system performance. The proposed approach was able to successfully detect the anomalies, with a low number of false positives (precision 90%-98%).

==> 2019_dsn_submitted/2019_dsn_content.tex <==
\section{Introduction}
\label{sec:intro}


%\toAA{Focus on Introduction}
% \toCG{\textbf{Intro main topics}:\\ virt/cloud: long adoption, but still a problem; }

%Problem statement and story line:

%What is the domain of applicability
%Why this is an important research question
%What is the state of the art
%What is our approach
%What are  the main  results presented in this paper and why are they  important?

%what is the paper overall goal?


%What is the domain of applicability:
%Anomaly Detection in Virtualized environments
%start with Virtual environments


%\vspace{-0.1in}
Virtualization environments enable the multiplexing of physical resources among many  virtual machines~\cite{barham_sigops2003xen, openstack_stories}. 
Cloud providers that use the \gls{iaas} model to share their infrastructure with multiple tenants rely on a  virtual machine manager,  also known as hypervisor~\cite{Tanenbaum2014}, to allocate physical resources to each virtual machine. 
Efficient, fair, and secure resource allocation approaches are critical aspects of the  IaaS model. 

%what is the problem - attacks
The ubiquity of cloud solutions~\cite{forbes_workload2020} is a potentially fertile ground for security and privacy breaches~\cite{intel, digitalocean, wallschlager2017automated, gulenko2016evaluating}. 
\textbf{In a multi-tenant environment, a legally acquired virtual host may initiate security attacks}, where a malicious user exploits hypervisor security vulnerabilities to attack a tenant that shares the same physical resources. 
Detecting and mitigating such attacks is an important step to counter the threat that such attacks pose to the existing IaaS systems and, more broadly, to the virtualization culture~\cite{hayes2008cloud}.

% \emph{Goals:} In this paper, we introduce a new methodology for anomaly detection based on the performance assessment of complex virtualized systems/environments, and we  show how this methodology overcomes some of the obstacles reported in the literature, among them, the high rate of false positives~\cite{Chandola2009}.

%%what is the proposed approach and related literature


%\emph{Challenges:}  % There is a vast literature on the analysis of the security aspects of cloud systems~\cite{Chandola2009,milenkoski2015evaluating}. % In~\cite{milenkoski2015evaluating}  the state of the art in intrusion detection systems (IDSes) was reviewed. Specifically,
% Milenkoski et al.~\cite{milenkoski2015evaluating}  reported that one of the most important open research questions in this domain is 

The design of intrusion detection systems (IDSs) for detecting zero-day attacks and advanced persistent threats (APTs)~\cite{GrottkeAMAA16} in virtualized environments poses several domain-specific challenges~\cite{Chandola2009,milenkoski2015evaluating}. 
%introduction to anomaly detection
In particular, $(i)$ it is challenging to comprehensively define normal behavior in a  diverse cloud environment, $(ii)$ malicious attackers may adapt their behavior to fit the domain definition of  ``normal behavior'', and $ (iii)$ data availability on anomalies at cloud environments, which would be instrumental for training purposes, is hard to obtain.  
To tackle those challenges, we focus on anomaly detection approaches based on system performance signatures. 
In particular, performance signatures have the potential of detecting zero-day attacks~\cite{Chandola2009,milenkoski2015evaluating}, as those approaches are based on detecting performance deviations and do not require detailed knowledge of attack history~\cite{FernandesJr2019}. 

% In addition, we show that  simple instances of the considered performance signature based  approaches   are amenable to  principled  model-based parameterization, allowing the system administrator to trade between multiple contending performance metrics. 

%%%Why anomaly detection is hard to implement
% \emph{Challenges:} In~\cite{Chandola2009} the authors have identified some of the obstacles to the successful implementation of anomaly  detection approaches in complex industrial systems, as the following:
% (i) it is very difficult to comprehensively define  normal  behavior, (ii) malicious  attackers  may  adapt their  behavior  to  fit  the  domain  definition  of  “normal  behavior'', (iii) anomaly  definition  varies  per  domain, (iv) data availability  for  anomaly  training  is  not  easy  to  obtain, (v) training  data  is  usually  noisy. 

%%%How the research presented in this paper addresses
%%these hard issues?. 
% As  a  consequence  of  these challenges, researchers usually develop heuristics for anomaly detection that take advantage of specific characteristics of the application domain. 

In this context, we pose  the following research question:  \textbf{is it feasible to efficiently tune  mechanisms for anomaly detection in complex virtualized systems},  trading between contending factors such as  the time to detect security attacks and the rate of false positives under a principled model-based framework?

%what is the data validation approach
%To validate the proposed approach we present an empirical assessment of anomaly detection effectiveness.

%%Introduce the methodology used in this paper
%We propose a methodology that tries to mitigate this.

In this paper, we \textbf{propose a methodology for anomaly  detection based on   performance deviations caused by security attacks in complex virtualized systems}.
%In particular, the proposed  methodology encompasses a principled 
%A model-driven approach is used to handle the high rate of false positives reported in previous works~\cite{Chandola2009}.
The proposed tuning of the anomaly detection mechanism leverages an analytical performance model and experimentation, and   allows to control the  rate of false positives in a principled manner~\cite{Chandola2009}.
After a careful analysis of every kind of transaction in the target system, the methodology profiles the system operation under normal conditions for its key transactions.
Then, during system operations performance monitoring,  performance deviations from the baseline are reported as security attacks.

%Experimental measurements in a controlled environment are used to assess the impact of attacks and tune the anomaly detection approach. 
To validate the proposed methodology, we ran an extensive experimental campaign employing the TPCx-V workload.  This workload  is representative of a large virtualized infrastructure that supports a business that relies on transactional systems.
Fault injection causing  system performance degradation emulates the effects of attacks impacting system performance.
Experience and practice show that injecting the effects of faults and attacks is an effective way to check systems tolerance to such faults and attacks~\cite{arlat1990fault, arlat2003comparison}.
System parameters tuning used measurements to trade between the rate of false positives and detection time of security intrusions.


The experiments showed the applicability and effectiveness of the proposed anomaly detection methodology.
In our experiments, it was possible to detect most of the performance deviations, with a low number of false positives. 
% ntensidade do failure mode é muito alta, o número de residual effects é maior ...

The methodology is also instrumental in identifying residual effects of attacks.
As expected, we observed more prominent transient residual effects after attacks that used more significant performance degradation  during the active attack period.  
Indeed,  stronger  attacks imply  longer recovery periods~\cite{nicol2004model, trivedi2009dependability}. 
%\nuno{The results show that our approach was able to successfully detect the anomalies, with a low number of false positives, and also spot possible residual effects on the system.}


Our proposal has the key advantage of being less intrusive than alternatives, e.g.,  that rely on deep packet inspection for monitoring and anomaly detection~\cite{FernandesJr2019,4579526,Wallschlager2017}.
In fact, it is \textbf{only necessary to monitor the throughput of the business transactions}, making it less dependant on the supporting technology stack and, therefore, more portable.
%In fact, it is \textbf{only necessary to watch the throughput of the business transactions}, making it less dependant on the supporting technology stack and, therefore, more portable.
Another main advantage is the anomaly detection algorithm simplicity,  which makes it easier to train, to understand, and to tweak than other algorithms that need complex learning processes.
These factors make the overall methodology easier to use and more applicable in practice.


%Focusing on measurements of business transactions;
%Focusing on throughput instead of response time;
%Use  experimental results to calibrate the analytical model and to be able to answer the following questions:
%What are the tradeoffs between rate of attacks and rate of false positive
%Formulate an optimization problem using as cost function the rate of false positives and security intrusions detection time
%What would have been the impact of selecting different BA tuning parameters
%We show experiments to validate this methodology.
%Using TPCx-V
%Using performance degradation faultload



In summary, the paper's contributions are the following:

$(i)$ A novel \textbf{anomaly detection methodology for detection of performance degradation attacks} based on the bucket algorithm and monitoring of the throughput of business transactions (Section~\ref{sec:meth}).

$(ii)$ An \textbf{analytical model to parameterize anomaly detection mechanism}, which allows conducting principled parameterization. The model can be used to cope with the tradeoff between time to detect an attack and the rate of false alarms (Section~\ref{sec:ad_algo}).

$(iii)$ An \textbf{experimental assessment  of the methodology in practice} using a representative system and attacks. We established the feasibility of detecting attacks based on non-intrusive user-level performance metrics that are available in production environments (Sections~\ref{sec:expEnvl}-\ref{sec:results}).

$(iv)$ A \textbf{model-driven principled mechanism design} that allows revisiting the experimental results and conduct what-if analysis to assess different performance metrics of the considered anomaly detection algorithms as a function of the parameterization (Section~\ref{ssec:modelbasedinsights}). 



% NAO TEMOS NADA DISTO :-)
%\textbf{Measurement campaign and insights:} we conduct a large scale measurement campaign to determine the impact of  attacks on the performance of virtualized services. 
%The campaign is executed using the TPCx-V workload,
% and serves to illustrate the applicability of  the proposed anomaly detection methodology. % (Section~\ref{sec:expCamp}).
%,  profiled during a set of executions.
%We selected a set of resource exhaustion attacks to emulate the effects of anomalies affecting system performance. 
%The results show that our approach was able to successfully detect the anomalies, with a low number of false positives, and also spot possible residual effects on the system.  
%
% -- and we show the feasibiity of parameterizing through the proposed model-based approach.
%
%

% The proposed  approach is  non-intrusive --  most of the data needed to support the approach is commonly available in production environments 



% \color{red}\nuno{Longo. Volto no fim corrigir, quando tiver uma ideia.}



The remainder of the paper is organized as indicated in the summary of contributions above.  
Section~\ref{sec:related} covers related work, followed by our contributions in Sections~\ref{sec:meth}-\ref{sec:results}. 
Section~\ref{sec:threats} covers threats to validity and Section~\ref{conc} concludes.

\begin{comment}
Section~\ref{sec:meth} introduces the new methodology for anomaly detection in complex virtualized environments, followed by the considered anomaly detection mechanism and its analytical model in Section~\ref{sec:ad_algo}. % In Section ~\ref{sec:ad_algo} we present the introduced heuristic for anomaly detection.
Sections~\ref{sec:expEnvl}-\ref{sec:results} describe the target system and the supporting infrastructure to conduct our experiments, along  with our  experimental results. % and  empirical  experimental results.%  In Section ~\ref{sec:results} we present the analysis of the obtained results. 
The model-driven parameterization of the anomaly detection mechanism is presented in Section~\ref{ssec:modelbasedinsights}.

\end{comment}
  % contains our conclusions and suggestions for future research. 
% The Appendix contains the  performance analysis of the anomaly detection approach  and  the related optimization problem.

\color{black}

\section{Related Work} 
\label{sec:related}

% \toCG{\na{Sinto o bg/rw curto para um paper deste género. É apenas um feeling, ainda não li.}\\
% \cg{Vamos atacar os pontos mais criticos, fechando a maior parte, ataco aqui. Entretanto vou pedir ao daniel para adicionar algo da parte analitica aqui.}}

%\cg{Should some of this ''Related work's´´ be spread throughout the work instead of being on this section ?}

%\toCG{Virtualization issues}
In this section, we revise  related  literature indicating how  the current work relates to  prior art.

%our research in the following domains: 

% (1) security issues related to cloud multi-tenancy, (2) IDS implementation using anomaly detection, (3)  anomaly detection using sequential hypothesis testing and (4) anomaly detection approaches using performance signatures.

%, and (5) metrics to benchmark security	vulnerability	detection	tools.

\subsection{Security issues related to cloud multi-tenancy} 

Multi-tenancy with isolation among tenants is the standard model  in cloud-computing  environments. 
However, regardless of the  hardware isolation mechanisms used, there have been many recently reported security intrusions  across these isolation barriers~\cite{Hunt2019}.  % An attacker co-located at the same physical host as the victim can create a security threat  by using a malicious virtual machine that can cause side-channels attacks, or even system resource exhaustion  causing a \gls{dos}~\cite{Gruschka2010,krishna2017virtualization}.
%
%
In~\cite{krishna2017virtualization, Gruschka2010},  the authors discuss security issues related to running the hypervisor in cloud environments. For example, a  malicious virtual machine running over the hypervisor could attempt to break the hardware isolation 
barrier, violate privacy rules or attempt to compromise the hypervisor, e.g., through a system resource exhaustion  causing a \gls{dos} attack. The papers also discuss  architecture features that would be needed to   mitigate these security vulnerabilities. In this paper, we focus on detecting anomalies in operational systems under the assumption that the aforementioned vulnerabilities cannot be fully prevented.   


 The tracking of system calls can be used to implement  Intrusion Detection Systems for virtualized environments~\cite{Alarifi2012}.  The idea consists of  watching, during execution,  for anomalous system call sequences in the user programs.   The assessment used a Linux KVM  virtual machine to collect the system calls from user programs. Results show a trade-off between detection result and time efficiency when comparing different system call sequence lengths.  Nonetheless, benchmarking the performance of IDS tools  is a challenging problem~\cite{antunes_metrics_2015}, motivating simpler and interpretable detection methods. Our work is complementary to~\cite{Alarifi2012}, as we indicate that IDS systems can benefit from  anomaly detection  approaches which are less intrusive than those reported in~\cite{Alarifi2012}, relying on~\cite{Alarifi2012} only on specific scenarios. 



% A key element of IDS systems are the  metrics monitored in real time.  In~\cite{antunes_metrics_2015}, the authors discuss	which metrics shall be used to benchmark security	vulnerability	detection	tools.	The	presented analysis showed that the	best metric	alternative	
% depends	on	the	usage	scenario.



\subsection{ Anomaly detection for cybersecurity} 

% :   hypothesis tests and performance signatures }

An approach for anomaly detection consists in running sequential hypothesis tests~\cite{ho2011fast,jung2004fast}.
In~\cite{jung2004fast},  sequential hypothesis tests are used for  the detection of malicious port scanners. The authors have developed a link between the detection of malicious port scans and the theory of sequential hypothesis testing. They have also shown that port scanning can be modeled as a random walk.  The detection algorithm matches the random walk to one of two  stochastic processes, which correspond to malicious remote hosts or to authorized remote hosts.  The approach considered in this paper is similar in spirit to that considered in~\cite{ho2011fast,jung2004fast}, as our analytical results are derived from a  birth-death Markov chain. Such Markov chain can be interpreted as a random walk  through buckets which fill as the system degrades, and empty as the system recovers (see Section~\ref{sec:analytmodel}).  


% The stochastic process classification is used to develop an anomaly detection algorithm, which was named TRW (Threshold Random Walk). The authors have shown that their anomaly detection algorithm only needs a small number of connection attempts   to detect malicious activity.
% The analysis of the anomaly detection algorithm stochastic behavior, allowed the authors to derive theoretical bounds on
% the probabilities of missed detection (false negatives) and false alarms (false positives).
%%compare to the \gls{ba} 
%%can we derive false negatives and false %% %% bounds positives using similar 

% \subsection{Anomaly detection  using performance signatures}


A number of previous works have considered anomaly detection approaches  using performance signatures~\cite{ Cherkasova2009, avritzer2010monitoring}. 
%
%\toCG{performance monitoring}
The work in~\cite{Cherkasova2009} introduces a framework that detects anomalous application behavior using regression-based models and application performance signatures. This method uses the concept of profiling  system resources, such as  CPU demand. Then,~\cite{avritzer2010monitoring} builds on top of~\cite{Cherkasova2009} and proposes an anomaly detection approach based on performance signatures based on CPU, I/O, memory and network usage   for the detection of security intrusions. The approach has been shown to  outperform, in some cases,  intrusion detection systems based on security intrusion history~\cite{milenkoski2015evaluating}.

The performance of signature-based intrusion detection systems rely on  intrusion detection algorithms that account for workload variability  to avoid a high rate of false positive alerts.  An example of such workload-sensitive algorithms is the \gls{ba}  that was introduced in~\cite{Avritzer2005} and is presented in detail in Section~\ref{sec:ad_algo}.
%presented in Section~\ref{sec:framework} and
% introduced in~\cite{Avritzer2005}.
%In addition, there is a need to detect baseline profile changes. 
Anomaly detection using the \gls{ba}  inspects the last sample of response time and compares it against the calibrated mean and standard deviation of response time. Then, it relies on the central limit theorem~\cite{AvritzerBGTW06} to assess if the last samples of response time comply with normal behavior or represent an anomaly. 
In Section~\ref{sec:ad_algo}  
we revisit the \gls{ba} mechanism, and present an analytical model that is instrumental to parameterize the \gls{ba} from experimental data.

% for anomaly detection in complex virtualized environments, and we revisit the 
% revisit the \gls{ba} mechanism, and.

%\toCG{metrics to detect anomalies}
% {\bf Metrics to benchmark security	vulnerability	detection	tools }


\setcounter{figure}{1} % aldrabice por causa das figuras

\begin{figure*}[!hb]
    \centering
    \vspace{-5pt}
    \includegraphics[width=0.9\linewidth]{./img/meth.pdf}
    \vspace{-5pt}
    \caption{Detailed representation of the methodology. We can observe three distinct sets of runs of the system: \textbf{E}xploratory, \textbf{P}rofile, and \textbf{V}alidation}
    \label{fig:meth}
\end{figure*}

    
    \section{Attack Detection Methodology} 
    \label{sec:meth}
    
This section describes the proposed attack detection approach, which has the goal of helping the users to successfully apply our anomaly detection algorithm into the life cycle of their systems. An essential aspect of an anomaly detection approach is to be able to cope with changes in the operational profile, as the monitored systems commonly have different loads and demands over time. 
Our methodology follows a cyclic approach and foresees additional iterations to accommodate each new operational profile.  
    \figurename~\ref{fig:meth_lc} depicts the high-level application of the methodology.
    
    \setcounter{figure}{0} % aldrabice por causa das figuras
    
    \begin{figure}[ht]
        \centering
        \includegraphics[width=\linewidth]{./img/meth_lc.pdf}
        \caption{Overview of the methodology application life cycle.}
        \label{fig:meth_lc}
        %\vspace{-5pt}
    \end{figure}
    
    \setcounter{figure}{2} % aldrabice por causa das figuras
    
    
    As we can observe, the methodology consists of three main phases: 
    \textbf{(A) exploratory analysis}, which allows determining the most effective way to monitor the system based on its characteristics; 
    \textbf{(B) profiling}, which evaluates the system on its expected regular operational profile(s)~\cite{Musa1993} to extract information about the habitual behavior and its performance;
    and \textbf{(C) Operation}, in which the system executes for its intended purposes, and we use all data and knowledge from the previous phases and report deviations, identifying them as anomalies or attacks. 
    
    A new iteration is needed if changes are detected: 
    $i)$ in the system, demanding a new complete iteration to see if there are relevant aspects to add to the monitoring surface,
    $ii)$ in the operational profile, requiring to repeat the profiling. This does not mean that the previous parameters are obsolete, it could represent a profile change that can be expected within some periodicity (e.g. holiday/promotion seasons). 
    
    The phases of methodology are detailed in  \figurename~\ref{fig:meth}, and explained in the ensuing sections.
    
    
    %An application of this method leads to a monitoring cycle that,  during the daily system operation ($C_{1}$), allows the user to detect attacks ($C_{2}$) by getting alerts ($C_{3}$) and take action ($C_{4}$) to establish the regular operation. 
    %Also, the methodology can be integrated into the system's life cycle and adapted to routinely incorporate the changes that occur in the system's operational profile. 
    
    
    
    
    \subsection{Exploratory analysis phase}
    
    This phase has the objective of determining the monitoring surface used to monitor the system's performance.  
    To achieve that goal, the user needs to follow three main steps:  
    
    $A.1)$ \emph{Analysis:} evaluate the system's internal aspects like its architecture, components, operations and resources that are available for monitoring to define how to characterize the system performance
     
    $A.2)$ \emph{Exploration:} the tacit knowledge of the system is essential, and a set of executions of the system (\textbf{E} on \figurename~\ref{fig:meth}) is prescribed for exploratory analysis. 
    During those executions,  all monitored data should be collected and analyzed  to understand the metrics that effectively translate into useful measurements;
    
    $A.3)$  \emph{Definition:} use previous steps to determine the \textbf{monitoring surface}. The monitoring surface analysis is the effort of joining the tacit knowledge and internal aspects to define which components and metrics to use in the following phases. 
    
    
    \subsection{Profiling phase}
    
    %\nuno{WiP: evaluate the environment under execution on its regular operational profile (a quantitative characterization of how a system will be used~\cite{Musa1993}) to extract information about the expected behavior and the optimal way of assessing the performance of the system}
    
    %  regular operational profile(s)
    
    This phase has the objective of evaluating the environment during the execution of its expected regular operational profiles~\cite{Musa1993}, in order to establish the statistical parameters that represent those profiles. 
    The following procedures are needed: 
    
    $B.1)$ \emph{Golden runs definition:} the system is exercised under usual operational conditions, i.e., without any fault/attack to collect the available data using the monitor surface. 
    These system's executions are called \textbf{golden runs} and are the primary reference for the system's normal behavior.  
    We split them into two independent sets: one \textbf{P}rofile set used to compute the baseline metrics, and the second set used to \textbf{V}alidate the performance parameterization.
    
     
    $B.2)$ \emph{Baseline metrics extraction:} the computation of the baseline metrics is conducted extracting statistical data from the metrics defined over the monitoring surface. 
    Those extractions should be made for each subsystem, metric, operation and resource, and operational profile. 
    
    % The computation of the baseline metrics is defined accordingly with the performance monitoring algorithm used.  Those metrics should be set for each subsystem, metric, transaction, and operational profile.
    
    % Once the baseline metrics are established, we are ready to calibrate the performance model using the empirical data generated. We run several experiments using the Golden Runs data and the detection algorithm with different configurations. The performance model determines which parameters are best suitable for the tests.  We, then, account for the number of alerts that a given setting will cause.  Since we are assessing experimental runs under no attack conditions, we can define the algorithm tolerance for the number of false positives accordingly with the user's threshold goal.  The performance model will assist in minimizing the false positive rate. The calibrated performance model is the algorithm parameterization that is best suitable for the system-specific detection goals.
    
    % The final step is the baseline validation to check the validity of the determined parameters. We run the detection algorithm with the Golden Runs from the \textbf{V} group and check if the number of alerts (false positives) is in the defined experiment criteria.  If this is not the case, we can go back to the recalibrate the performance model until the requirements are fulfilled.
    
    
    $B.3)$ \emph{Performance model calibration:} apply the empirical data to determine the optimal values that minimize the false positives (FP) alerts. 
    The performance model determines which parameters are best suitable for the tests.  
    Then, we account for the number of alerts that a given setting will cause.  
    As we are assessing experimental runs under no attack conditions, we can define the algorithm tolerance for the number of FPs according to the user's preference.
    The performance model will assist in minimizing the FP rate. 
     
    $B.4)$ \emph{Baseline validation:} check the validity of the determined parameters. Apply the detection algorithm using the Golden Runs from the \textbf{V} group and check if the number of alerts (FP) is in the defined experiment criteria.  
    
    $B.5)$ \emph{Parameterization adjustment:}  during the baseline validation, if the alert rate does not meet the defined objective, we can go back and recalibrate the performance model until the requirements are met.
    
    
    
    \subsection{Operation phase}
    \label{sec:met_op}
    
    % \nuno{wip: Finally, on the Operation step, we use all data and knowledge from the previous components to search for anomalies or attacks during the system operation. }
    
    At this point, the anomaly detection algorithm is fully configured to monitor the system in production and detect security attacks that cause performance degradation. 
    Thus, in this phase, we take advantage of all the data and knowledge from the previous components to search for anomalies or attacks during the system operation.
    We need to:
    
    $C.1)$ \emph{Define a criterion:} that determines an alert condition in a concise manner. For instance, every alarm in any transaction or only alerts in critical subsystems?
    
    $C.2)$ \emph{Monitor the operation:} integrate the detection algorithm into the daily activity by continually watching  the monitoring surface using the detection algorithm with the optimal parameters
    
    
    
    


\section{Anomaly Detection Mechanism and Model} 
\label{sec:ad_algo}

In this section we describe the anomaly detection mechanism used in the proposed methodology and also the principled analytical model used. 

\subsection{Anomaly detection mechanism} 

%\toCG{ainda fala muito de response time}

The algorithm for anomaly detection heuristic based on performance degradation works by continuously  estimating  the mean response time, $\overline{x}$, and maintaining 
$B+1$ buckets of depth $D$ each, which contain  the  history of the most recent response times, as shown in \figurename~\ref{intrusion}. %The R notation is used to represent the point estimate of system response time.  
$P$ is a pointer to the
current bucket and $d$ is the number of recent response
time samples stored in the current bucket. 

Let $\mu$ be the baseline average response
time, and  $\sigma$ be the baseline standard deviation. Both $\mu$ and $\sigma$ can be  
derived from the execution of  the controlled  experiments (\textbf{golden runs}). The pointer $P$ to the current bucket is used to determine the current estimate of the average response time, which is given by  $\overline{x} = \mu + P  \sigma$. Once the current bucket overflows (resp., underflows), the algorithm estimate of the current average response time is shifted upward (resp., downward) by one standard deviation.  When all buckets overflow a performace degradation is detected and 
when all buckets underflow the system has recovered from a transient performance degradation. 

The performance degradation detection algorithm, that we will refer hereinafter as just Bucket Algorithm (\gls{ba}), is given as follows:

%\begin{enumerate}
\emph{Initialization:} $\{P\leftarrow 0; d\leftarrow 0 \}$, with all buckets empty.
 
\emph{Main loop:} for each sample $\hat{x}$ of response time, execute the steps below.
    
\begin{enumerate}
\item  if $P > B$, all buckets overflow, trigger performance degradation alarm;
\item if $\hat{x} > (\mu + P \sigma)$ then $\{ d \leftarrow d + 1 \}$,  response time larger than reference value, add token to the current bucket;
\item else do $\{ d \leftarrow d - 1\}$,  response time smaller   or equal than reference value, remove token from the current bucket;
\item if $(d > D)$ then do $\{ d \leftarrow 0; P \leftarrow P+1 \}$, current bucket overflow, go to next bucket;
\item if $\big((d < 0)$ and $(P >0)\big)$ then
do $\{ d \leftarrow D; P\leftarrow P-1\}$,  current bucket underflow,  go to previous bucket;
\item  if $\big((d < 0)$ and  $(P == 0)\big)$ then
do $\{d \leftarrow  0\}$ all buckets empty, system recovered from transient performance degradation.
\end{enumerate}
% \end{enumerate}

\begin{figure}
    \includegraphics[width=1\linewidth]{bucketsgraffle} \vspace{-0.2in}
    \caption{System of buckets diagram representing the dynamics of the detection algorithm. %, showing $B$ buckets of depth $D$ each. $P$ is the pointer to the current bucket and $d$ is the number of recent response times stored in bucket $P$.  Note that a buffer underflow indicates recovery from transient performance degradation, while the overflow of the last bucket triggers a security alarm.
    $D$ and $B$ must be properly parameterized for each operation}
    \label{intrusion}
    \vspace{-0.1in}
\end{figure}


The performance degradation detection algorithm can be tuned by varying the bucket depth, $D$, and the number of buckets, $B$.  The larger the product $D\times B$  the longer it takes  for the algorithm to detect the performance degradation. 
%However, shorter times of $D\times B$, would lead to a larger fraction of false positives. 
The statistical analysis  of the behavior of this family of \glsplural{ba} has been described on~\cite{AvritzerBGTW06}.


\subsection{Analytical model motivation and goals}



%\subsubsection{Motivation}

Sequential probability ratio test~\cite{jung2004fast} and the bucket algorithm~\cite{AvritzerBGTW06} are used to detect attacks in networks.  
Their analysis involves a random walk birth-death process.  
In the bucket algorithm, for instance, in the initial state all buckets are empty, and in the final state all buckets are full.  
Understanding the mean time to reach the final state, one can tune the number of buckets and the depth of each bucket in a principled way. 
%
%In this appendix, we present some preliminary ideas on the principled tuning of the bucket algorithm.  We envision that those preliminary ideas can be combined with recent advances in the study of birth-death processes (e.g.,~\cite{jouini2008moments}) to yield more refined results.
%
Simple algorithms to detect attacks, such as the bucket algorithm, can be tuned using first principles.


%\subsubsection{Goals}


%How does the depth of the bucket impact the probability of false positives?  
The larger the depth of the bucket, the lower the false positive probability, but the longer it takes for a true positive to be identified.
To simplify the analysis, we \textbf{work under the assumption} that attacks will change the response time distribution, and will always be detected.
However, the number of samples to detect the attack may vary depending on the depth of the bucket.
Our \textbf{second key simplifying assumption is} that the number of samples to detect the attack is much smaller than the number of samples collected before getting a false positive (which should be always the case in practice: the time until a false positive should be much longer on average than the time until a true positive).  

Then, we aim at answering the following question: what is the smallest bucket depth to produce a false positive probability bounded by a given threshold?

\subsection{Analytical model}
\label{sec:analytmodel}

Next, we introduce a 
discrete time birth-death Markov chain (DTMC) to characterize the behavior of the \gls{ba}. State $(b,d)$ of the Markov chain corresponds to the setup wherein there are $d$ balls in bucket $b$, and $D$ balls in buckets $b-1, \ldots, 1$.


Each  transition of the DTMC corresponds to the collection of a new sample. 
Such sample   causes the system to transition from state $(b,d)$ to one of its two neighboring  states. 
Let  $p_i$  be the probability that the number of balls at bucket $i$ increases after a new sample is collected.  
Then, $p_i=\mathbb{P}(\hat{x}  > \overline{x} + (i-1)\sigma),$ for  $ 1 \leq i \leq B$. 
The entries of the transition probability matrix are readily obtained from \figurename~\ref{fig:dtmc}, with the explicit expression of the transition probability matrix is presented in~\cite{techreport}.


\begin{figure}[ht]
    \centering
    \includegraphics[width=1\columnwidth]{newbucketdiagram.pdf}
    \caption{Discrete time Markov chain characterizing the behavior of the \gls{ba}.  Each transition corresponds to the collection of a new sample.}
    \label{fig:dtmc}
\end{figure}



  %given as follows:

\begin{comment}
  
  \begin{align}
     & p_{(k,d),(\tilde{k},\tilde{d})}= \\
      &\left\{
      \begin{array}{lll}
      P(\hat{x}  > \overline{x} + k\sigma), & \textrm{if } & (d < D, \tilde{d} = d+1,  k=\tilde{k}) \textrm{ or }   \\
             & &( d = D, \tilde{d} = 1,  k-1=\tilde{k} )  \textrm{ or } \\           &  & (d = D, k = K,      \tilde{k} = \textrm{absorbing})   \\
              P(\hat{x}  \leq \overline{x} + k\sigma), & \textrm{if } & (d > 1, \tilde{d} = d-1,  k=\tilde{k}) \textrm{ or }   \\
             & &( d = 1, \tilde{d} = D,  k+1=\tilde{k} )  \textrm{ or } \\           &  & (d = \tilde{d}= 0, k =\tilde{k}= 1),   \\
             0, & \multicolumn{2}{l}{\textrm{otherwise.}}   
      \end{array}\right.
 \nonumber \end{align}

\end{comment}
 
Once the terminal absorbing state  is reached  an alarm is triggered. The DTMC is illustrated for the case $B=2$ in \figurename~\ref{fig:dtmc}. 
The number of samples collected until absorption  accounts for a tradeoff between the mean time until $(a)$ a  false alarm, in the absence of attacks, and $(b)$ detection, in the presence of an attack.  Larger values of bucket depth  $D$ favor the reduction of the former but  increase the latter. 
 
Let $A_B(p_1,p_2,D)$ be the mean time until absorption, measured in number of collected samples, accounting for $B$ buckets of depth $D$ each. 
We derived a closed-form~\cite{techreport} expression for the time until absorption, which  is instrumental to handle that tradeoff.
In particular, for $B=2$, the resulting expression is given by
%
%Let $A_2$ be the time to absorption with $K=2$ buckets.   $A_2$ can be expressed as a function of $p_1$, $p_2$ and $D$,
\begin{align}
A_2(p_1,p_2, D)  %V_{D+1,1,0} + V_{D,2,1} \\
&= A^{(1)}_2(p_1,p_2, D)  + A^{(2)}_2(p_1,p_2, D) \label{eq:a2p1p2d}
\end{align}
where $A^{(i)}_B$ is the mean time to fill the $i$-th out of $B$ buckets,
\begin{align}
A^{(1)}_2 &=   { \Delta_1} \left(\delta_1- D\right) \\
A^{(2)}_2 %&=  \left( \frac{1+\rho_2}{1-\rho_2} + U_{0,2} \right)  \left(\frac{1-\rho_2^{-D}}{1-\rho_2^{-1}} \right) - D \frac{1+\rho_2}{1-\rho_2}   \\
% &=  \left( \Delta_2 + \Delta_1\frac{1-\rho_1^{D+1}}{\rho_1^{D+1}}\right)  \left(\frac{1-\rho_2^{-D}}{\rho_2-1} \right) - D \Delta_2 \\
&=  \Delta_2\left( \delta_2
-D\right) + \Delta_1\left(\frac{1-\rho_1^{D+1}}{\rho_1^{D+1}}\right)  \delta_2
\end{align}
%\begin{align}
%U_{0,2} 
%   &= \frac{1}{1-p_2} \left(1 + p_2  (\rho_1+1)\frac{\rho_1^{-D-1}-1}{1-\rho_1} \right) % \\
    % &=\frac{1+\rho_1}{\rho_1} \frac{1-\rho_1^{-n}}{1-\rho_1^{-1}} + \rho_1^{-n} ({1+\rho_1^{-1})}  
%\end{align}
and
\begin{equation}
    \rho_i = \frac{1}{p_i} -1, \qquad \Delta_i=\frac{1+\rho_i}{1-\rho_i}, \qquad \delta_i = \frac{1-\rho_i^{-D}}{\rho_i-1}.  
\end{equation}


% In what follows, we numerically illustrate the behavior of the quantities of interest and the subsumed tradeoff.

% \toCG{Notation Table ? \nuno{sera necessario?} \cg{Sugestão do daniel, disse muito comum, mas acho que podemos passar, só checar a consistência.} }

% \toCG{Check consistency over the paper K in the modeling would be the B in the empirical study \nuno{ja esta? ja nao acho K} \cg{Fazendo o double check! Removo o comentario em breve}}



\subsection{Parameterization of the anomaly detection mechanism:  a model-driven optimization approach}
\label{sec:param_ad}

\subsubsection{Why model-driven parameterization?}
 To compare different configurations of the \gls{ba} , we face the problem that the increase of $B$ or $D$ changes the detection sensitivity and time to alert.  

 To illustrate this phenomena, let us simplify the problem and consider that the system's transactions happens in a fixed interval time $t$. 
Assuming a critical workload, where all samples $\hat{x}$ (transactions) evaluated are always greater than the $(\mu + P \sigma)$, the minimum amount of time to detect any anomaly has a length of $BDt$. 
 For that reason, the number of maximum alerts within any time-specific $l$ is determined by $\frac{l}{BDt}$. That way, for another distinct configuration, if $B$ or $D$ increases, the number of possible alerts will decrease. 


 For that reason, the consideration of what defines a detection or its absence should be defined accordingly with the application and system. 



\subsubsection{Hypothesis testing}

The system administrator continuously considers two alternative hypothesis:  $(i)$ null hypothesis $H_0$ corresponding to a situation where there is no attack taking place
and $(ii)$ alternative hypothesis $H_1$ meaning that the system is under attack. Then, the key quantities of interest can be defined as a function of $H_0$ and $H_1$.

\begin{definition}
The  mean time until a false alarm under $H_0$ is denoted by $A_B$.  It is given by the mean time to  reach the absorbing state of the Markov chain characterizing the bucket algorithm.
\end{definition}



\begin{definition}
A lower bound on the  time until a true positive  under $H_1$  is denoted by $L$.  Assuming all buckets are initially empty, we let $
    L = BD$.
\end{definition}

\begin{definition}
The probability of false alarm is the probability that an alarm is triggered outside an attack,
$  f = \mathbb{P}(R < T), $ 
where $R$ is a random variable with mean $A_B$ characterizing the time until an alarm is triggered,  and  $T$ is  a random variable with mean $1/\alpha$ characterizing the time until an attack occurs.
\end{definition}


In this paper, except otherwise noted we assume that $f$ depends on $R$ and $T$ only through their means, i.e., $f = f(A_B, \alpha^{-1})$.



\begin{definition} \label{def:cost}
The expected cost of a given system parameterization is a weighted sum of the probability of false positives, computed under $H_0$,  and a lower bound of the time until detecting an attack, computed under $H_1$,
 \begin{equation}
     C(\bm{p}, w, D, B, \alpha)  =  B D +  w f(A_B, \alpha^{-1})  \label{eq:cost1}
 \end{equation}
\end{definition}



\subsubsection{Modeling the probability of false alarms} 
We assume that attacks arrive according to a Poisson process with rate $\alpha$. 
Let $f$ be the probability of a false alarm.  We consider two distinct models to determine the probability of false alarm as a function of $A_2$ and $\alpha$. The deterministic  (resp., exponential) model  presumes that  the number of samples taken until a false alarm can be well  approximated by  a deterministic (resp., exponential) distribution with mean  $A_2$.  
 Then,
\begin{equation}
    f = \varphi(A_2 \alpha) 
\end{equation}
\begin{comment}
\begin{equation}
    f = \varphi(A_2 \alpha)  e^{- A_2 \alpha} \label{eq:fexp1}
\end{equation}
and
\begin{align}
    f = \frac{1/A_2}{\alpha + 1/A_2}  =  \left( 1+{A_2}{\alpha} \right)^{-1} \label{eq:fexp2}
\end{align}
\end{comment}
where $\varphi(x) = e^{-x}$ and $\varphi=1/(1+x)$
under the deterministic and exponential models, respectively.


\subsubsection{Optimization problem formulation} \label{sec:optimization}

Given a target false positive probability, denoted by $F$, the system administrator goal is to  determine the optimal number of buckets and bucket  depth so as to 
minimize the lower bound on number of samples to detect and attack, $L$, while still meeting the target false positive probability. 
\begin{align}
&{\mbox{\sc  Problem with Hard Constraints:}}\quad  \nonumber \\
&    \min \quad L=BD \\ \label{eq:hard}
 &   \textrm{subject to} \quad f(B,D) \leq F  
\end{align}
In what follows, we assume that $B$ is fixed and given.  Then, as $f$ is strictly decreasing with respect to $D$, the constraint above will be always active and the problem translates into finding the minimum value of $D$ satisfying the constraint.  The problem above is similar in spirit to a Neyman-Pearson hypothesis test, for which similar considerations apply, i.e., the optimal parameterization of the test is the one that satisfies a constraint on the false positive probability.  

Alternatively, the problem above can be formulated through the corresponding Lagrangian, 
\begin{align}
&{\mbox{\sc  Problem with Soft Constraints:}}\quad \nonumber  \\
& \min     \mathcal{L}(D) = B D + w (f(B,D)- F)  \label{eq:lag} 
\end{align}
where $w$ is the Lagrange multiplier.  The Lagrangian naturally leads to an alternative formulation of the problem, wherein  the hard constraint in~\eqref{eq:hard} is replaced by a soft constraint corresponding to the penalty term $f(B,D)- F $ present in the cost Lagrangian. The Lagrangian is a cost function, motivating Definition~\ref{def:cost}. Note that as $wF$ is a constant, minimizing~\eqref{eq:lag} is equivalent to minimizing~\eqref{eq:cost1}.

\begin{comment}
Note that whereas the {\mbox{\sc  Problem with Hard Constraints}} is defined as a function of the target false alarm probability $F$, the {\mbox{\sc  Problem with Soft Constraints}}   is defined as  a function of the weight $w$.  Although there is a mapping between the two problems, the target false alarm probability may be easier to interpret as it has a concrete physical interpretation as opposed to $w$, which is a Lagrange multiplier.  Nonetheless, the cost function defined by $w$ allows to visually determine the value of $D$ that minimizes cost. For this reason, the two formulations may be complementary, as indicated in the upcoming section through a numerical example parameterized using data from our controlled experiments. 

\end{comment}

\section{Experimental Validation} 
\label{sec:expEnvl}

To demonstrate and validate the methodology described in Section~\ref{sec:meth}, we defined an experimental study that uses the \gls{tpcxv}, which is representative of complex systems that take advantage of virtualization to support businesses, as presented in Section~\ref{ssec:sut}.
The operational phase is emulated through a series of runs of the benchmark in which we inject a set of faults that emulate the effects of attacks that affect system performance, as explained in Section~\ref{ssec:faults}. 
We go over all the phases  to apply the proposed methodology, describing the main considerations and the key data obtained in each step, including the performed exploratory analysis in Section~\ref{ssec:sut-exploratory},
the profiling phase in Section~\ref{ssec:sut-profiling}, the operational phase in Section~\ref{ssec:sut-operational}, and the model calibration in Section~\ref{ssec:modelbasedinsights}.



\subsection{System Under Test} 
\label{ssec:sut}

The typical virtualization environment that is representative of a real-world scenario of cloud computing providers, can be quite complex and have many properties that are difficult to emulate in a practical testbed.  
In this work, we are interested in a compromised multi-tenant cloud computing infrastructure, which is composed by several users sharing this infrastructure, one of which trying to exploit the vulnerabilities present on the underlying hypervisor.    



The \gls{tpcxv} is a public available, end-to-end benchmark for data-centric workload on virtual servers. The benchmark kit provides the specification,  implementation, and tools to audit and run the benchmark. Details can be found in~\cite{tpcv2013, tpcv2015}.
It models many features commonly present in cloud computing environments such as multiple \glspl{vm} running at different load demand levels, and significant fluctuations in the load level of each \gls{vm}~\cite{tpcv2013}.  
We use the workload and software provided by the \gls{tpcxv}\cite{tpcv2015} to emulate a context closely related to a real-world scenario of brokerage firms that must manage customer accounts, execute customer trade orders, and be responsible for the interactions of customers with financial markets.

\figurename~\ref{fig:tpc-arch} shows the transaction flow. 
The virtual client emulator (vce), interacts with the different brokerage firms (distinct groups), which in turn communicates with the virtual market emulator (vme). 
%may be viewed as a Data Center in a Box'' as it 
\gls{tpcxv} uses virtualization technology to co-locate database tiers and application-management tiers on logically distinct \glspl{vm} within a single computer system.

%\figurename~\ref{fig:businesmodel} illustrates the different entities modeled by the \gls{tpcxv} and the related transactions among them. 

% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.9\linewidth]{./img/transFlow_v2.pdf}
% \caption{ \scriptsize Business Model Transaction Flow}
% \label{fig:businesmodel}
% \end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=.9\linewidth]{./img/tpc-arch.png}
    \caption{TPCx-V components and transactions flow (from~\cite{TPCx-V_spec}). In this work, each group is treated as distinct subsystem. } 
    \label{fig:tpc-arch}
\end{figure}

The goal of \gls{tpcxv} is to measure how a virtualized server runs database workloads, using them to measure the performance of virtualized platforms, specifically the hypervisor, the server hardware, storage, and networking. The minimal deployment of the \gls{tpcxv} will have four groups, each with three \glspl{vm}, representing different subsystems that contribute differently for the overall load during the {\bf{}}  { \bf{ \texttt{10} distinct load phases} of \texttt{12} minutes}  that exist during a typical run. 
The different components of \gls{tpcxv} are architecturally distributed as depicted in \figurename~\ref{fig:tpc-arch}

The \gls{tpcxv} workload is made up of \textbf{\texttt{12} types of transactions} with different characteristics that are submitted for processing at multiple databases (market, customer, and broker) following a specified mix of transactions for different phases. 
Transactions are used to simulate the stock trade process, and when a trade finishes, a transaction name \textit{Trade-Result} is issued. 
The primary performance metric for the benchmark works as a business throughput and is known as \texttt{tpsV}, and portrays the number of completed \textit{Trade-Result} per second.


%Additionally to the specification, the benchmark kit comes with a set of software components with its implementation and tools to audit and run the benchmark. 
%Discussion about experimental performance metrics, design considerations,  tunning deployments, and others practicals considerations of the \gls{tpcxv} are present in~\cite{tpcv2013, tpcv2015}.  


Our \textit{experimental setup} is a deployment of the \gls{tpcxv} over two physical servers. The first, a Dell PowerEdge R710 with 24 Cores, 96 GB RAM, and 12 TB disk, managed by a Xen hypervisor (4.4.1), has a privileged domain (dom0), and 17 virtual machines with different configurations, a set dedicated to the \gls{tpcxv} and other that will represent our compromised tenants. Another server, with 2 Core, 8GB RAM and 1 TB disk, with the same hypervisor, host the \gls{vm} driver component into a different host as prescribed on the \gls{tpcxv} specification. The details of each \gls{vm} is described in \tableautorefname~\ref{tab:vms_spec}.

As we can see in the \tableautorefname~\ref{tab:vms_spec}, the resources specifications varies for each group (tpc-g\textit{n} refers for a \gls{vm} for group \textit{n}) and it was defined following the recommendations on~\cite{TPCx-V_spec}.  Since a group is a set o three \gls{vm}, our malicious user will have access to the same amount of \glspl{vm}. 


\begin{table}[t]
\centering
\caption{ \scriptsize  \glspl{vm} name, memory and the number of virtual CPUs. The tpc-driver is supported on a different physical host}
\label{tab:vms_spec}
\vspace{-0.05in}
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{ccc||ccc||ccc}
\toprule

\textbf{\gls{vm} } & \textbf{MB}  & \textbf{vCPU}   & \textbf{\gls{vm}} & \textbf{MB}  & \textbf{vCPU}  & \textbf{\gls{vm}} & \textbf{MB}  & \textbf{vCPU}     \\ \midrule
tpc-g1a         &   1024    & 1  & tpc-g2b2        &   6144    & 6  & tpc-g4b1        &   20400   & 2 \\
tpc-g1b1        &   8192    & 2  & tpc-g3a         &   1024    & 1  & tpc-g4b2        &   10240   & 8 \\
tpc-g1b2        &   4096    & 4  & tpc-g3b1        &   16384   & 2  & tenant A        &   1532    & 2 \\
tpc-g2a         &   1024    & 1  & tpc-g3b2        &   8192    & 8  & tenant B        &   1532    & 2 \\
tpc-g2b1        &   12288   & 2  & tpc-g4a         &   1024    & 2  & tenant C        &   1532    & 2 \\ \midrule
dom0            &   1962    & 4  & tpc-driver\footnotemark[1]      &   1882    & 2 & & &\\ 
\bottomrule
\end{tabular}
%\vspace{-0.15in}
\end{table}

We developed tools to trigger all tests, start benchmark components, report any problem during the test, and manage all the interactions between the environment, benchmark, and tests.  
Each \textbf{single experiment lasts roughly 4 hours} that correspond to the 2h demanded as minimum by the benchmark specification, and another 2h to restore the system.
These tools restore the environment to the same initial state to ensure the reproducibility across different experiment runs. 
It does this action basically by rebooting the servers and recovering the system and databases (restoring all virtual disks).







% \begin{table}[ht]
% \small
% \centering
% \caption{ \scriptsize \glspl{vm} resource specifications}
% \label{tab:vms_spec}
% \begin{tabular}{@{}ccc@{}}
% \toprule
% \textbf{\gls{vm} name} & \textbf{Memory(MB)}  & \textbf{vCPU}      \\ \midrule
% dom0            &   1962    & 4 \\
% tpc-g1a         &   1024    & 1 \\
% tpc-g1b1        &   8192    & 2 \\
% tpc-g1b2        &   4096    & 4 \\
% tpc-g2a         &   1024    & 1 \\
% tpc-g2b1        &   12288   & 2 \\
% tpc-g2b2        &   6144    & 6 \\
% tpc-g3a         &   1024    & 1 \\
% tpc-g3b1        &   16384   & 2 \\
% tpc-g3b2        &   8192    & 8 \\
% tpc-g4a         &   1024    & 2 \\
% tpc-g4b1        &   20400   & 2 \\
% tpc-g4b2        &   10240   & 8 \\
% tenant A        &   1532    & 2 \\
% tenant B        &   1532    & 2 \\
% tenant C        &   1532    & 2 \\ \midrule
% tpc-driver\footnotemark[1]      &   1882    & 2 \\ \midrule
% \bottomrule
% \end{tabular}
% \end{table}
% \footnotetext[1]{Supported on a different physical host}






\subsection{Fault Model}
\label{ssec:faults}



The fault model used in our work explores one of the possibles attack models on cloud computing: the resource exhaustion pattern~\cite{Gruschka2010}.  In this kind of attack, the virtual guest can obtain more resource than allowed or even lead the system into a Denial-of-Service state. 
They can be divided into two main categories~\cite{Groza2011}: 
i) \textit{excessive use}, where there is no abnormal use, but the consumption of resources is significantly higher than the others; and 
ii) \textit{malicious use}, where the intentional abuse of the resources lead the system to a failure state.

Since the \gls{tpcxv} has a database workload, an attack that explores the primary resources used in these systems will surely have an impact on the performance and, consequently, the reference metric of the system.
To the best of our knowledge, we are unaware of a real exploit tailored for virtual environments that focus explicitly on the hypervisor and tries to exhaust the typical resources used on database services. 

To overcome the absence of a representative attack, we simulated a resource exhaustion behavior by using the Stress-NG software~\cite{stressng}, which was designed to ``exercise various physical subsystems of a computer as well as the various operating system kernel interfaces'' and can be parameterized to perform many IO and CPU operations in various forms. 
We defined three configurations to emulate our attack and test our system:  

 \textit{(H):}  A High-Intensity workload: during 300 seconds it starts eight processes to abuse the system IO;
 
 \textit{(L):} A Low-Intensity workload: during 300 seconds, we perform ten intervals of 15 seconds of IO-abuse and 15 with no workload.  The workload uses two IO stressors processes;
  
 \textit{(Ls):} Shorter Low-Intensity workload: the same as the (L) configuration but with only three intervals.
  






We defined the duration of the configuration based on proportional time of the \gls{tpcxv} run, roughly 4\% and 1\%. The configurations length are also less than the benchmark phase (\texttt{12} min, as explained in Section~\ref{ssec:sut}). The number of IO process was defined empirically, running different configuration and checking which one did not freeze the Guest-VM or was not too small to do not be considered abusive. We will reference those configurations as H, L, and Ls, respectively.

% \toNA{Think about the testing name : change the 6 and 4 for a more significant name : \toCG{maybe we can just name the test when it is on the peak performance and non-peak performace...  It will be P and nP ... PH \textit{P}L \textit{nP}Ls}}


Since the \gls{tpcxv} has different phases with diverse load demands (see Section~\ref{ssec:sut-operational}), we focused the attack on two distinct phases, on the \texttt{4th}, which is when \textbf{the group with more physical resources has a more significant contribution to the overall load}  and the \texttt{6th}, when \textbf{the reference metric achieves the highest rate}. 

Combining those two definitions, we have a total of \texttt{6} fault models, which we will refer to using the phase plus the configuration reference: \texttt{4H}, \texttt{4L}, \texttt{4Ls}, \texttt{6H}, \texttt{6L}, and \texttt{6Ls}.






\subsection{Exploratory Phase}
\label{ssec:sut-exploratory}

The first part was to understand the  \gls{tpcxv} architecture, and its specification to get some tacit knowledge about its deployment in our environment.  
In previous works~\cite{AvritzerBGTW06,avritzer2010monitoring},  the \gls{ba} was applied using response time as the anomaly detection metric. 
In this work, we are evaluating a complex system with different components and subsystems that aims to maximize its throughput. 
Hence, we decided to also use the system's throughput as the input metric for the \gls{ba}.   

Based on the response time data available from the \gls{tpcxv} results, we derived a throughput extraction process that aggregates the transactions by group, phase, transaction type, and  the operation completion time. 
Also, to accommodate a metric that is best when its value is short (contrary to the response time), we changed the algorithm to invert the logic. 
It will penalize the metric if its value is lower than the average plus a multiple of the standard deviation, i.e., $\hat{x} < (\mu + P \sigma)$.

The next step was to perform several exploratory runs, that allowed to conduct a characterization of every transaction and applied the \gls{ba} in all data collected to make a preliminary assessment. 
The analysis revealed that not all of the \gls{tpcxv}'s transactions are useful in reflecting the system's load. 
Additionally, the results from the response time evaluation showed an higher variability that leads to a higher number of false alarms.

Concluding the exploratory phase, we defined our monitoring surface as the throughput information of \texttt{9} (of the \texttt{12}) transactions from \gls{tpcxv}. 
That data will be evaluated distinctly for every subsystem (the \texttt{4} \gls{tpcxv}'s groups), resulting in \texttt{36} (\texttt{9x4}) bucket algorithms running, each with \texttt{10} distinct configurations, \texttt{1} for each distinct operation profile (the \texttt{10} \gls{tpcxv}'s phases). 


% After evaluating the algorithm using both metrics, we rapidly noticed that by using the throughput data, we have better results as \tableautorefname~\ref{tab:rtVsTput} shows.  Additionally, some results are different. For instance, in the run 595 (6H), we did not alert in the injection period using the RT, but it did report using the throughput database.

% \begin{table}[ht]
% \normalsize
% \centering
% \caption{Performance comparison for b=2 and d=15}
% \label{tab:rtVsTput}
% \begin{tabular}{cccc}
% \toprule
% & \textbf{TP} & \textbf{FP} & \textbf{Precision\footnotemark[1]} \\ \midrule
% Response Time & 182 & 522 & 25,85\% \\
% Throughput & 1874 & 38 & 98,01\% \\ 
% \bottomrule
% \end{tabular}
% \end{table}
% 
% \footnotetext[1]{For this precision account we simply counted the number of alerts inside and outside the attack period.}


\subsection{Profiling Phase}
\label{ssec:sut-profiling}

To profile the system, we executed 59 golden runs to generate data for the characterization of the system's baseline behavior (37 runs, {\it P set}) and also validation (22 runs, {\it V set}).  
For every transaction from the monitoring surface, we compute and store the average throughput for each subsystem in every operational profile.   
These values are the system's baseline metrics. 

To calibrate our performance model (Section~\ref{ssec:modelbasedinsights}), we need to account for the following metrics:  
\begin{enumerate}
    \item The probability of a false positive alarm as a function of bucket depth;
    \item The probability for each transition in the DTMC (\figurename~\ref{fig:dtmc});
    \item The mean time to first alarm during an attack.
\end{enumerate}

To compute those probabilities, we applied the \gls{ba} with different configurations over the {\it V set} runs data. 
These results are presented in Section~\ref{sec:results}.

For the validation process, we applied the \gls{ba} for every golden run, accounting for the number of alerts (false positives). 
The goal of this step is to check if using the parameters suggested by the model will not generate an unacceptable amount of false-positive alerts.
First, we execute the assessment with the same runs used to generate the baseline metrics ({\it B set}). 
Here we are not validating, only producing values to compare later with the validation results.  
Also, this step can use for consistency check and test for possible computational errors if the results show any abnormal number of alerts. 
Then we repeat the process using the validation runs ({\it V set}). 
The results of both sets are not significantly different, and thus we present only the validation values in~\tableautorefname~\ref{tab:basel_param}.

We can see in \tableautorefname~\ref{tab:basel_param} that using two buckets is more effective, as it shows a fair number of false-positive alerts. 
One bucket has too many alerts, and three is likely to be ineffective.

\begin{table}[ht]
%\small
\vspace{-0.1in}
\centering
\caption{\scriptsize  False positive alerts: total count and average ($\mu$) by run in validation}
\label{tab:basel_param}
\vspace{-0.05in}
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{cccc||cccc||cccc}
\toprule
\textbf{B} & \textbf{D} & \textbf{\# Alerts} & \boldmath$\mu$  
& \textbf{B} & \textbf{D} & \textbf{\# Alerts} &  \boldmath$\mu$ 
& \textbf{B} & \textbf{D} & \textbf{\# Alerts} & \boldmath$\mu$  \\\midrule

1 & 30 & 27373 & 1244,23 & 2 & 12 & 4 & 0,18 & 2 & 21 & 0 & 0,00 \\
2 & 6 & 185 & 8,41 & 2 & 15 & 0 & 0,00 & 3 & 10 & 0 & 0 \\
2 & 9 & 12 & 0,55 & 2 & 18 & 0 & 0,00 & & & & \\\bottomrule
\end{tabular}
\end{table}


Looking at the \tableautorefname~\ref{tab:basel_alert_txns}, we can see that for distinct transaction types, we have distinct sensitiveness for the same parameterization when applying the \gls{ba}.  These distinct sensitivities can suggest that different values for $D$ should be applied for different operations.

\begin{table}[ht]
%\small
\vspace{-0.1in}
\centering
\caption{\scriptsize  False positive alerts segmented by \gls{tpcxv}'s transactions }
\label{tab:basel_alert_txns}
\vspace{-0.05in}
\begin{tabular}{cc|ccccccccc}
\toprule
\multicolumn{2}{c|}{ \textbf{Transaction ID} } & 0 & 1 & 2 & 4 & 5 & 6 & 7 & 8 & 9 \\
\midrule
\multirow{3}{*}{ \textbf{D} } & 6 & 23 & 43 & 28 & 34 & 12 & 23 & 14 & 2 & 6 \\
& 9 & 0 & 1 & 4 & 6 & 1 & 0 & 0 & 0 & 0 \\
& 12 & 0 & 0 & 2 & 2 & 0 & 0 & 0 & 0 & 0 \\\bottomrule
\end{tabular}
\end{table}


When running the \gls{ba} in both golden runs sets, we obtain similar results. This similarity indicates that the profile derived from the baseline metrics generalizes for different runs.

After the previous analyses, we were able to apply the performance model in the experimental data. Section~\ref{ssec:modelbasedinsights}  details the complete process. The calibrated performance model suggests $D \in (12,15]$, and the number of alerts withing this range is acceptable. 




\subsection{Operational Phase}
\label{ssec:sut-operational}

%In this experimental campaign, we will adapt the methodology operation step to perform an empirical study of the \gls{ba} applicability.

As prescribed in Section~\ref{sec:met_op}, we have to define our alert criterion.  
We adopted distinct approaches to detect \textit{true positives} (TP) and \textit{false positives} (FP).  
A TP is when we detect {\bf at least one alert on the attack phase}. 
We only need one alert in any group for any transaction type. 
Complementarily, a \textit{False Negative} (FN) is when \textbf{no alert is raised} on the same phase.  
We consider an FP \textbf{every bucket overflow that happen in the no-attack phase}. 
In this case, two bucket overflows in distinct transactions, or even in the same, but in different groups, will account for two distinct FP. 
This approach is justified as in any detection system, a better tool is the one that is effective and minimizes the number of false positives. 

An alert on the post-attack phase can be an FP or either a residual effect caused by the faultload. 
For that reason, we cannot assert exactly anything about it, but we will discuss this further in Section~\ref{sec:re}.

At last, the \textit{true negative} (TN) is not necessary to be defined.  
The problem is that the \gls{ba}  is designed to detect a deviation from the regular operation continuously during its execution.  
To estimate the number of possible alerts during a specific period, based on a fixed detection window, does not make sense when comparing different workloads and configurations (see Section~\ref{sec:param_ad}).

During the testing campaign process, each of our test runs is composed of three phases, as depicted in \figurename~\ref{fig:testDesc}.  
In those periods defined, we will count the number of FP, TP, and FN as described early. 
Each alert on the post-attack phase will count as a {\it residual effect}.  
When executing the \gls{tpcxv} workload, we will run just one attack, as defined in Section~\ref{ssec:faults}. 
As showed in \tableautorefname~\ref{tab:runs}, we performed 21 runs for each fault injection type, while applying the \gls{ba} throughout the monitoring surface.

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{./img/test_desc_v2.pdf}
    \caption{Distinct phases and its alerts meaning during a test run.}
    \label{fig:testDesc}
\end{figure}

\begin{table}[ht]
    \vspace{-0.1in}
    %\small
    \centering
    \caption{Runs in Experimental Campaign}
    \label{tab:runs}
    \vspace{-0.05in}
    \begin{tabular}{c||cccccc||c}
    \toprule
    Test & 4H & 4L & 4Ls & 6H & 6L & 6Ls & Golden \\
    $N^{o}$ Runs & 21 & 21 & 21 & 21 & 21 & 21 & 59 \\\bottomrule
    \end{tabular}
\end{table}


After the test executions, we used the data collected to apply the \gls{ba} with different parameterizations to study the effectiveness of the method. 
An initial observation, based on the data presented in previous analysis and  \tableautorefname~\ref{tab:bd_variat}, is that the optimal number of buckets is two.
But which specific configuration is more effective in which failure mode are demonstrated in the next section.


\begin{table}[b]
    %\normalsize
    \centering
    \caption{\scriptsize Fraction of attack alerts over all alerts varying $B$ and $D$. We are accounting all alerts, not following the detection's criterion.}
    \label{tab:bd_variat}
    \vspace{-0.05in}
    \setlength\tabcolsep{3pt} % default value: 6pt
    \begin{tabular}{ccr|ccr|ccr|ccr}
    \toprule
    \textbf{B} & \textbf{D} & \textbf{\%} & 
    \textbf{B} & \textbf{D} & \textbf{\%} & 
    \textbf{B} & \textbf{D} & \textbf{\%} & 
    \textbf{B} & \textbf{D} & \textbf{\%} \\\midrule
    1 & 30 & 7,71\% & 2 &  9 & 97,40\% & 2 & 15 & 98,01\% & 2 & 21 & 97,62\% \\
    2 & 6 & 92,22\% & 2 & 12 & 97,74\% & 2 & 18 & 98,01\% & 3 & 10 & 0,00\% \\\bottomrule
    
    \end{tabular}
\end{table}

\subsection{Model Assisted Calibration of Anomaly Detection} 
\label{ssec:modelbasedinsights}


This section provides insights on the experimental results using the proposed model to define the best parameterization based on system's data.
First, we parameterize the proposed model  from  the experimental data. 
To exemplify the general process, we focus on  the  TRADE\_LOOKUP transaction, for which we  identify  that $p_1$ and $p_2$ equal 0.46 and 0.71, respectively. 
We assess the expected number of samples until a false alarm, obtained from~\eqref{eq:a2p1p2d}, with  $B=2$, $p_1=0.46$,  $p_2=0.71$, and letting $D$ vary between 1 and 30.  For $D=15$, we observed that the number of samples until a false alarm surpasses  $10^7$. 

% \figurename~\ref{fig:modelpar1} is obtained 

\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{bucketfig1.png}
    \caption{Expected number of samples until false alarm,  derived from the proposed analytical model.
    We note that  for $D=15$ the number of samples until a false alarm surpasses   $10^7$.} \label{fig:modelpar1}
\end{figure}

\end{comment}

\begin{figure}[t]
    \centering
    %\includegraphics[width=0.4\textwidth]{prob_fp.pdf}
    \includegraphics[width=\linewidth]{img/prob_fp.pdf}
\caption{Probability of false alarm from model tuned based on  experiments.}
%When $D=12$ the probability of false alarm is already close to 0.}
\label{fig:modelpar2}
\end{figure}

\begin{comment}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{plot4.png}
    \caption{ Cost as a function of bucket depth $(D)$.  Cost is given by $C=w f+ K D$, with $K=2$ and $w=909$, where $f$ is the probability of false alarm. Under the deterministic (resp., exponential) model, cost is minimized for $D=13$ (resp., $D=18$). }
    \label{fig:modelpar3}
\end{figure}

\end{comment}


\figurename~\ref{fig:modelpar2} % and~\ref{fig:modelpar3} 
accounts for an attack model, wherein the mean time between  attacks is $1/\alpha=5 \times 10^5$ samples, i.e., the attack rate is  $\alpha=2 \times  10^{-6}$ attacks per sample.   As the bucket depth increases, the probability of false alarm decreases.   For $D  \ge 12$, the probability of false alarm is  close to 0.

As discussed above, there is a tradeoff between the probability of false alarm and the time to detect attacks once they occur.  To cope with such a tradeoff, we consider both approaches  introduced in Section~\ref{sec:optimization}, namely the hard and soft constraint problems.  
Under the hard constraint problem,  a target probability of false alarm is determined, and the minimum value of $D$ that satisfies such target is sought.  For instance, if we set $F=0.03$ in~\eqref{eq:hard} then the minimum value of $D$ satisfying the constraint is $D=15$ and $D=13$ under the exponential and deterministic attack models, respectively.


\begin{comment}
a simple cost function, which is given by a weighted sum of two terms.  The first term corresponds to the probability of false alarm  and the second  corresponds to the  number of samples necessary to detect an attack once it occurs,  
\begin{equation}
    C(\bm{p}, w, D, K, \alpha)  = f(A_B, \alpha^{-1}) + w K D
\end{equation}
where $w$ is a weight balancing between the two contending aspects.

\end{comment}

We also assess how the cost  $C(\bm{p}, w, D, B, \alpha)$ introduced in Definition~\ref{def:cost}  varies as  a function of $D$,  letting $B=2$, $p_1=0.46$, $p_2=0.71$ and $\alpha=2 \times  10^{-6}$.  Letting $w=909$, which corresponds to the Lagrange multiplier of the constrained problem under the deterministic model (see also~\eqref{eq:lag}),  the optimal bucket depth equals $D=13$, %.  Considering the same parameterization, the optimal bucket depth equals  $D=18$ under the  exponential model,
which is in agreement with the result  presented in the previous paragraph.  Note that for the exponential model the minimum cost is attained at $D=18$, which is slightly larger than $D=15$ obtained in the previous paragraph. This is because the Lagrange multiplier corresponding to the exponential model is $w=57$.  Using such a smaller weight  favors a reduction in the optimal bucket depth to $D=15$, again in agreement with the results discussed in the previous paragraph.  

% depending on whether the deterministic or exponential   models are used  to determine the probability of false alarm as a function of $A_2$.   

\emph{Take away message and engineering implications:}
the analysis presented in this section is instrumental to perform what-if counterfactual analysis and execute utility-driven model parameterization.  If the system administrator implements global countermeasures against attacks, for instance, it is expected that the rate of attacks will decrease. In that case, the bucket depth can be adjusted accordingly, e.g., using the proposed utility-driven approach presented in this section.


% The approach can be initially configured through the mechanism previously illustrated, and then tuned to account  for novel system  setups.


\begin{comment}
Next, we discuss some engineering implications derived from our model-driven analysis of the experimental results.

\textbf{Reverse engineering utility function of existing systems}  
The results presented in this section are instrumental to reverse engineer the utility function subsumed by existing systems.  For instance, consider a system operating with $B=2$ buckets with depth $D=15$. The analysis presented in the previous section shows that this is optimal, for instance, in case $5\times 10^{5}$ samples are collected inbetween attacks and $w=57$, leading to a false positive probability of roughly 0.03.   Knowing that this is the case, one can tune the utility function, e.g., to account for attacks that occur at different rates, and verify when/if the parameters of the bucket algorithm should be adjusted.

\textbf{Counterfactual analysis} As pointed in the previous paragraph, reverse enginneering the utility function is helpful to perform what if analysis and execute utility-driven model parameterization.  If the system administrator implements global countermeasures against attacks, for instance, it is expected that the rate of attacks will decrease. In that case, the bucket depth can be adjusted accordingly, e.g., using the proposed utility-driven approach presented in this section. The approach can be initially configured through the reverse engineering mechanism previously illustrated, and then tuned to account  for novel system  setups.


\end{comment}

\begin{comment}

\clearpage
\pagebreak

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.4\textwidth]{bucketfig1.png}
    
       (a) Expected number of samples until false alarm,  derived from the proposed analytical model.
    We note that   for $D=15$ the number of samples until a false alarm surpasses   $10^7$.
    
    \includegraphics[width=0.4\textwidth]{bucketfig2.png}

(b) Probability of false alarm, under exponential and deterministic models. In both cases, when $D=15$ the probability of false alarm is already close to 0.  

    \includegraphics[width=0.4\textwidth]{bucketfig3.png}
    
    (c) Cost as a function of bucket depth $(D)$.  Cost is given by $C=f+0.018 D$, where $f$ is the probability of false alarm. Under the exponential model, cost is minimized for $D=15$. 

    \caption{    Analytical results derived from parameterized model, letting $K=2$, $p_1=0.46$ and $p_2=0.71$. In parts (b) and (c),  we let the attack rate be given by  $\alpha=2 \times  10^{-6}$ attacks per sample. }
    \label{fig:apfig1}
\end{figure}

\end{comment}



\color{black}


\section{Results and Discussion}
\label{sec:results}

In this section, we first analyze the residual effects that can arise after the attacks and how to identify them. Following, we carry out the analysis of the effectiveness of the anomaly detection approach using two case studies in our environment. 

Our results are discussed using three metrics widely adopted in classification assessment~\cite{zaki2014dataminingbook}, namely  precision, recall and F-measure, which are defined as a function of true positives (TP), false positives (FP) and false negatives (FN) as follows,

\begin{small}
\begin{align}
\textrm{Pr} = \frac{TP}{TP + FP},  \ \ &
\textrm{Re} = \frac{TP}{TP + FN},    &
\textrm{F1} = \frac{2 \times \textrm{Pr} \times \textrm{Re}}{\textrm{Pr} + \textrm{Re}}.  
\label{eq:perf_equa} 
% &= \frac{2 \times TP}{2\times TP + FN + FP}
\end{align}
\end{small}

Precision (Pr) measures the impact of FP in the method's positive prediction.
Recall (Re)  reflects the sensitiveness of the algorithm, capturing the fraction of corrected predictions. 
 F-measure (F1) is the harmonic mean of precision and recall,  balancing them in a single metric. 
 
 % Equation~\eqref{eq:perf_equa} define those metrics.
%
% tirei as virgulas porque pareciam apostrofos na formula anterior


% \label{eq:precision}

\subsection{Residual Effects}
\label{sec:re}

During our experimentation we observed that the number of alerts immediately after the attack phase was significantly higher than in other non-attack period.
We carried an analysis to understand what does it mean the alerts that appear in the post-attack phase.  
We accounted for the number of alarms and the distance, in seconds, from the end of the attack injection phase. 
As \figurename~\ref{fig:re} shows, most of the bucket overflown happens a few seconds after the attack, which suggests that those alerts can be residual effects and not false positives.  

\begin{figure}[htb]
\centering
\vspace{-0.05in}
\includegraphics[width=\linewidth]{./img/alerts_residual.pdf}
\vspace{-0.1in}
\caption{Post-attack alerts distribution for bucket configuration with B=2 and D=[12,15]. Note that x scale is cropped to simplify for more readability.}
\label{fig:re}
\vspace{-0.05in}
\end{figure}

A natural question that arises is what is a reasonable threshold that would discriminate between false positive and residual effects of the attack.  
Regression techniques,  outliers detection techniques, among others, can be used to estimate that threshold. 
In this work, to calculate a reasonable limit without increasing the complexity, we computed the meantime for the first alarm during the attack phase. 
We used it as a threshold estimation to differentiate residual effects from FP.  

In \tableautorefname~\ref{tab:re_thrsd}, we can see the meantime to first attack for two transactions for different bucket's depth. 

\begin{table}[ht]
 %\small
\centering
\vspace{-0.05in}
\caption{ \scriptsize Mean time to first alarm during the attack injection (in seconds)}
\label{tab:re_thrsd}
\begin{tabular}{ccccc}
\toprule
\textit{\textbf{Transaction}} & \textbf{d=6} & \textbf{d=9} & \textbf{d=12} & \textbf{d=15} \\\midrule
TRADE\_LOOKUP & 31,03 & 50,06 & 69,18 & 61,63 \\
MARKET\_WATCH & 36,08 & 54,11 & 60,38 & 59,51 \\\bottomrule
\end{tabular}
\end{table}


We know that, on average, the number of seconds to the \gls{ba} alarm over some constrains (parameters and transaction) is $\delta$.  
We also know that an attack has just ended. 
So, it is reasonable to assume that any alert that occurs in time $t < \delta$  can be associated with residual effects (emptying queues, recovering from errors states, etc.)  of the previous attack, and that is our reasoning behind this approach.


\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{./img/residual_effects.pdf}
    
    \caption{Distribution of the residual effects by failure mode and bucket depth.}
    \label{fig:re_breakdwon}
    \vspace{-0.05in}
\end{figure}


\figurename~\ref{fig:re_breakdwon} shows additional evidences that corroborate with our assumption. 
Only the failure mode with higher (H) intensity induce those alerts. 
When the system is in its peak performance, phase six (blue dashed line), the number of alerts is greater than in the fourth phase. 
Finally, when $D$ increases, the number of alerts decreases, what is expected if those alerts are related to residual effects, since the larger the $D$, the bigger is the tolerance for transient faults.

\vspace{-0.06in}
\subsection{Case Study 1}

In our first case study, we will assess the detection effectiveness of the \gls{ba} over our fault models and how the parameterization affects the method's performance. 
Here we will use the same parameterization for all operations.
The optimal $D$ value, accordingly with our calibrated model, resides between 12 and 15. 
\tableautorefname~\ref{tab:cs1_tbl} shows the metrics our tests, segmented by different failure modes, and for {\it ALL} failure modes mixed. 

\begin{table}[ht]
    \tiny
    \vspace{-0.1in}
    \centering
    \caption{Metrics values for $D=(12|15)$ of CS1. Maximal value for \textbf{TP} would be 21 for each failure mode and 126 for \textbf{ALL}. }
    \vspace{-0.1in}
    %Table also shows the Residual Effects counts (\textbf{RE}) and \textbf{Pr}ecision, \textbf{Re}call and F-measure (\textbf{F1}) metrics}
    \label{tab:cs1_tbl}
    \includegraphics[width=0.9\linewidth]{./img/cs1_tbl.pdf}
    
\end{table}


The first observation from \tableautorefname~\ref{tab:cs1_tbl} is the method's low number of alerts outside of an attack.  Since we count every alert as an FP, the possibles number of this category could be much higher since we are accounting $4\times 9$ buckets at the same time.  Following, we can note that the \gls{ba} is not useful, in general,  for short attacks with low-intensity, the except is the 6Ls at $D=12$, but it has a worse result compared with the others failure modes. Conversely, to others failure-modes, the method is very effective, even with an f-measure of 1 for the 6H at $D=12$. 


% \begin{figure}[htb]
% \centering
% \includegraphics[width=\linewidth]{./img/precision.pdf}
% \caption{ \scriptsize 
% Campaign Precision for all falt models using two buckets. The data are shown with the  pre and pos phases splitted into two sets.}
% \label{fig:precision}
% \end{figure}


\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{./img/all_metrics.pdf}
\caption{Campaign Precision for all falt models using two buckets. The data are shown with the  pre and pos phases splitted into two sets.}
\vspace{-0.2in}
\label{fig:all_metrics}
\end{figure}

Another question that we tried to answer is what is the impact of the bucket depth on the target metrics (Equation~\ref{eq:perf_equa})? \figurename~\ref{fig:all_metrics} shows the results. Reinforcing our previous observation, the \textit{Ls} failure mode do not perform and are responsible for the small values on those charts. 

A general observation that we can get from the Precision and Recall charts in this analysis is that those metrics have different relations with the bucket depth.  Precision increases with $D$ as the Recall decreases. In this case, the F-measure is an excellent way to balance the method's efficiency. Comparing the different bucket depth, the precision and recall will vary for the distinct failure modes.

% 
% \begin{figure}[htb]
% \centering
% \includegraphics[width=\linewidth]{./img/recall.pdf}
% \caption{ \scriptsize Campaing Recall for two bucket configuration}
% \label{fig:recall}
% \end{figure}



Considering that, ideally, a method should work for every kind of attack, in this case study, $D=12$ provides better results (All curve). But obviously, this is not the case for every system, and one should balance the parameters to get ideal performance, which reinforces the importance of our analytical model and tuning the method by each transaction. 


% \begin{figure}[htb]
% \centering
% \includegraphics[width=\linewidth]{./img/f_measure.pdf}
% \caption{ \scriptsize F-Measure across the different fault models for both phases under evaluation.}
% \label{fig:f1}
% \end{figure}

\subsection{Case Study 2}

We have seen in \tableautorefname~\ref{tab:basel_alert_txns} that not every transaction has similar configuration. A natural assumption is that different parameterization for each operation should lead to better performance.  To validate that intuition, based on the cited table, we created a mix (Mix 6/9/12/15) of parameterization in which we use the first null $D$ value for each transaction. \tableautorefname~\ref{tab:cs2_tbl} show the results. 

Despite being a better positive predictive setup, it almost tripled the number of FP which greatly penalize the overall performance of the configuration. Those transactions with lower bucket depth cause this higher number of FP. 


\begin{table}[ht]
    \tiny
    \centering
\caption{ \scriptsize Result of Case Study 2, showing the Residual Effects counts (\textbf{RE}), \textbf{Pr}ecision, \textbf{Re}call and F-measure (\textbf{F1}) metrics}
    \label{tab:cs2_tbl}
    \includegraphics[width=0.9\linewidth]{./img/cs2_tbl.pdf}
\end{table}

As a next tunning, following our analytical model, we avoided the values of $D$ below 12, just raised the values of 6 and 9 to 12. The results are, also shown on \tableautorefname~\ref{tab:cs2_tbl}.  

In general, the performance is increased, especially for the {\it L} cases. The exception is the {\it Ls} failure mode, that we already now that are not well covered by the method. 






\section{Threats to Validity}
\label{sec:threats}

% \toNA{\cg{Nem tudo ai pode fazer sentido, estou so fazendo um brainstorm para depois iterar sobre}}

Next, we discuss some of the  assumptions considered in this paper and their implications. 

 \emph{Fault model representativeness}: %  as in any experimental exercise, we had to trade between simplicity and representativeness. To that aim, we considered a database  workload, namely the TPCx-V benchmark.  Then, 
 the faults injected in the system are  generated by stressing the underlying OS. In real systems, different attacks may produce various effects on multiple layers of the system stack.  Nonetheless, as far as the subsumed OS states resulting from those attacks correspond to states generated by our fault injection, the  considered failures are representative of those that occur in  systems under operation~\cite{arlat1990fault, arlat_dependability_2002}. 
 
%  For that reason, one can argue about the representativeness of those faults.   But this limitation is minimized since the observed state of the system characterizes a 
 
 
\begin{comment}
 
 
  \emph{Target environment and workload}: As in any experimental exercise, we had to trade between simplicity and representativeness. To that aim, we considered a database  workload, namely the TPCx-V benchmark.  We envision that our experiments can be easily extended to other workloads, and leave that as subject for future work. %  and some of its related metrics the throughput capacity and is not generic.
 
 \emph{Assessment at scale}: we consider system-wide global detection of anomalies. Alternatively, one can consider  segmented anomaly detection for subsystems inside the considered ecosystem.  The nuts and bolts of how to combine the results of multiple anomaly detection instances per subsystem are out of the scope of this work, although such assessment is contemplated  by  the proposed methodology.  
 
\end{comment} 
 
%  thus restrict the applicability. Nevertheless, such an assessment is possible within this methodology.
  
  \emph{Profile obsolescence:} if user profiles are not stable,  %if the operational profile changes, 
  the number of false alerts can increase significantly, making the detection system useless until the next iteration. In that case, time must be divided into windows and the solution presented in this paper needs to  be applied and tuned at every  window.  To determine the optimal window size  one may rely on techniques for learning in non-stationary environments~\cite{sayed2012learning}.
  
  
  
%  can be challenges for some systems that do not have a stable operational profile. 
  
  %  \emph{Obsolescence}: if the operational profile changes, the number of false alerts can increase significantly, making the detection system useless until the next iteration.

 \emph{Covert degradation}: single metrics  may not suffice to detect anomalies.  A detector  using response time as its metric, for instance,  may miss-detect attacks that impair  system availability if the few transactions that succeed to  complete have their response time within  the expected  range.  A similar effect occurs  with respect to  throughput in elastic systems. This limitation can be mitigated using multiple complementary metrics for anomaly detection.





\section{Conclusion} 
\label{conc}

In this work, we presented a methodology for anomaly detection based on performance degradation caused by security attacks for complex virtualized systems.  The approach leverages an analytical model to optimize the detection technique in a principled way. % and was designed to allow  integration into the daily operation and adapt to system's changes.  
Our experimental assessment indicates the method's effectiveness by  injecting resource exhaustion attacks in a complex virtualized system. Results show that it is possible to detect anomalous behavior using  the throughput of the business transactions with an average precision of 90\% and recall of 86\%.  Our experimental results also bring awareness about residual effects of  high-intensity fault loads, which may persist for a significant amount of time after the active attack has been interrupted. Such residual effects  give rise to false positives,  further motivating the use of analytical models to  tune the false positive rate in a principled  fashion.

% During our experimental campaign, we were able to differentiate the residual effects of high-intensity fault loads.




==> 2019_dsn_submitted/commentTools.tex <==
\usepackage{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{soul}
\usepackage{graphicx}
 \usepackage[hidelinks]{hyperref}
% \AfterPreamble{\hypersetup{
%   hidelinks
% }}


\definecolor{mauve}{rgb}{0.58,0,0.82}
\definecolor{armygreen}{rgb}{0.29, 0.33, 0.13}
\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}

\newboolean{showcomments}
\setboolean{showcomments}{true}% TODO set false to disappear

\ifthenelse{\boolean{showcomments}}
{\newcommand{\mynote}[3]{\fbox{\bfseries\sffamily\tiny#1}% no space
{\scriptsize$\blacktriangleright$\textsf{\color{#3}{#2}}$\blacktriangleleft$}}}
{\newcommand{\mynote}[3]{}}

\newcommand{\na}[1]{\mynote{NA}{#1}{red}}
\newcommand{\nuno}{\na}
\newcommand{\antunes}{\na}
\newcommand{\mv}[1]{\mynote{MV}{#1}{mauve}}
\newcommand{\charles}[1]{\mynote{CG}{#1}{armygreen}}
\newcommand{\cg}{\charles}
\newcommand{\avz}[1]{\mynote{AA}{#1}{blue!50}}
\newcommand{\alberto}{\avz}
\newcommand{\beto}{\avz}
\newcommand{\daniel}[1]{\mynote{DM}{#1}{green}}

\newcommand{\toNA}[1]{\todo[inline, color=red!70]{\fbox{\bfseries\sffamily\scriptsize NA} #1}}
\newcommand{\toMV}[1]{\todo[inline, color=mauve!70]{\fbox{\bfseries\sffamily\scriptsize MV} #1}}
\newcommand{\toCG}[1]{\todo[inline, color=asparagus]{\fbox{\bfseries\sffamily\scriptsize CG} #1}}
\newcommand{\toAA}[1]{\todo[inline, color=blue!50]{\fbox{\bfseries\sffamily\scriptsize Alberto} #1}}
\newcommand{\toDM}[1]{\todo[inline, color=green]{\fbox{\bfseries\sffamily\scriptsize DM} #1}}


\newcommand{\wut}[0]{\fcolorbox{red}{white}{\bfseries\sffamily\tiny{\tiny$\blacktriangleleft$\textsf{\scriptsize\color{red}{(?)}}}}}
\newcommand{\MR}[0]{\fcolorbox{blue}{green}{\bfseries\sffamily\scriptsize{\small$\blacktriangleleft$\textsf{\color{blue}{REF}}}}}
%todo inline
\newcommand{\actionitem}[1]{\todo[inline]{\fbox{\bfseries\sffamily\scriptsize TODO} #1}}
%todo NOTE:
\newcommand{\note}[1]{\todo[inline, color=gray!10]{\fbox{\bfseries\sffamily\scriptsize Note} #1}}
%\newcommand{\note}[1]{\todo[inline, color=gray!10]{\fbox{\bfseries\sffamily\scriptsize Note} #1}}


==> 2019_dsn_submitted/content.tex <==
\section{Introduction}
\label{sec:intro}


%\toAA{Focus on Introduction}
% \toCG{\textbf{Intro main topics}:\\ virt/cloud: long adoption, but still a problem; }

%Problem statement and story line:

%What is the domain of applicability
%Why this is an important research question
%What is the state of the art
%What is our approach
%What are  the main  results presented in this paper and why are they  important?

%what is the paper overall goal?


%What is the domain of applicability:
%Anomaly Detection in Virtualized environments
%start with Virtual environments


%\vspace{-0.1in}
Virtualization environments enable the multiplexing of physical resources among many  virtual machines~\cite{barham_sigops2003xen, openstack_stories}. 
Cloud providers that use the \gls{iaas} model to share their infrastructure with multiple tenants rely on a  virtual machine manager,  also known as hypervisor~\cite{Tanenbaum2014}, to allocate physical resources to each virtual machine. 
Efficient, fair, and secure resource allocation approaches are critical aspects of the  IaaS model. 

%what is the problem - attacks
The ubiquity of cloud solutions~\cite{forbes_workload2020} is a potentially fertile ground for security and privacy breaches~\cite{intel, digitalocean, wallschlager2017automated, gulenko2016evaluating}. 
\textbf{In a multi-tenant environment, a legally acquired virtual host may initiate security attacks}, where a malicious user exploits hypervisor security vulnerabilities to attack a tenant that shares the same physical resources. 
Detecting and mitigating such attacks is an important step to counter the threat that such attacks pose to the existing IaaS systems and, more broadly, to the virtualization culture~\cite{hayes2008cloud}.

% \emph{Goals:} In this paper, we introduce a new methodology for anomaly detection based on the performance assessment of complex virtualized systems/environments, and we  show how this methodology overcomes some of the obstacles reported in the literature, among them, the high rate of false positives~\cite{Chandola2009}.

%%what is the proposed approach and related literature


%\emph{Challenges:}  % There is a vast literature on the analysis of the security aspects of cloud systems~\cite{Chandola2009,milenkoski2015evaluating}. % In~\cite{milenkoski2015evaluating}  the state of the art in intrusion detection systems (IDSes) was reviewed. Specifically,
% Milenkoski et al.~\cite{milenkoski2015evaluating}  reported that one of the most important open research questions in this domain is 

The design of intrusion detection systems (IDSs) for detecting zero-day attacks and advanced persistent threats (APTs)~\cite{GrottkeAMAA16} in virtualized environments poses several domain-specific challenges~\cite{Chandola2009,milenkoski2015evaluating}. 
%introduction to anomaly detection
In particular, $(i)$ it is challenging to comprehensively define normal behavior in a  diverse cloud environment, $(ii)$ malicious attackers may adapt their behavior to fit the domain definition of  ``normal behavior'', and $ (iii)$ data availability on anomalies at cloud environments, which would be instrumental for training purposes, is hard to obtain.  
To tackle those challenges, we focus on anomaly detection approaches based on system performance signatures. 
In particular, performance signatures have the potential of detecting zero-day attacks~\cite{Chandola2009,milenkoski2015evaluating}, as those approaches are based on detecting performance deviations and do not require detailed knowledge of attack history~\cite{FernandesJr2019}. 

% In addition, we show that  simple instances of the considered performance signature based  approaches   are amenable to  principled  model-based parameterization, allowing the system administrator to trade between multiple contending performance metrics. 

%%%Why anomaly detection is hard to implement
% \emph{Challenges:} In~\cite{Chandola2009} the authors have identified some of the obstacles to the successful implementation of anomaly  detection approaches in complex industrial systems, as the following:
% (i) it is very difficult to comprehensively define  normal  behavior, (ii) malicious  attackers  may  adapt their  behavior  to  fit  the  domain  definition  of  “normal  behavior'', (iii) anomaly  definition  varies  per  domain, (iv) data availability  for  anomaly  training  is  not  easy  to  obtain, (v) training  data  is  usually  noisy. 

%%%How the research presented in this paper addresses
%%these hard issues?. 
% As  a  consequence  of  these challenges, researchers usually develop heuristics for anomaly detection that take advantage of specific characteristics of the application domain. 

In this context, we pose  the following research question:  \textbf{is it feasible to efficiently tune  mechanisms for anomaly detection in complex virtualized systems},  trading between contending factors such as  the time to detect security attacks and the rate of false positives under a principled model-based framework?

%what is the data validation approach
%To validate the proposed approach we present an empirical assessment of anomaly detection effectiveness.

%%Introduce the methodology used in this paper
%We propose a methodology that tries to mitigate this.

In this paper, we \textbf{propose a methodology for anomaly  detection based on   performance deviations caused by security attacks in complex virtualized systems}.
%In particular, the proposed  methodology encompasses a principled 
%A model-driven approach is used to handle the high rate of false positives reported in previous works~\cite{Chandola2009}.
The proposed tuning of the anomaly detection mechanism leverages an analytical performance model and experimentation, and   allows to control the  rate of false positives in a principled manner~\cite{Chandola2009}.
After a careful analysis of every kind of transaction in the target system, the methodology profiles the system operation under normal conditions for its key transactions.
Then, during system operations performance monitoring,  performance deviations from the baseline are reported as security attacks.

%Experimental measurements in a controlled environment are used to assess the impact of attacks and tune the anomaly detection approach. 
To validate the proposed methodology, we ran an extensive experimental campaign employing the TPCx-V workload.  This workload  is representative of a large virtualized infrastructure that supports a business that relies on transactional systems.
Fault injection causing  system performance degradation emulates the effects of attacks impacting system performance.
Experience and practice show that injecting the effects of faults and attacks is an effective way to check systems tolerance to such faults and attacks~\cite{arlat1990fault, arlat2003comparison}.
System parameters tuning used measurements to trade between the rate of false positives and detection time of security intrusions.


The experiments showed the applicability and effectiveness of the proposed anomaly detection methodology.
In our experiments, it was possible to detect most of the performance deviations, with a low number of false positives. 
% ntensidade do failure mode é muito alta, o número de residual effects é maior ...

The methodology is also instrumental in identifying residual effects of attacks.
As expected, we observed more prominent transient residual effects after attacks that used more significant performance degradation  during the active attack period.  
Indeed,  stronger  attacks imply  longer recovery periods~\cite{nicol2004model, trivedi2009dependability}. 
%\nuno{The results show that our approach was able to successfully detect the anomalies, with a low number of false positives, and also spot possible residual effects on the system.}


Our proposal has the key advantage of being less intrusive than alternatives, e.g.,  that rely on deep packet inspection for monitoring and anomaly detection~\cite{FernandesJr2019,4579526,Wallschlager2017}.
In fact, it is \textbf{only necessary to monitor the throughput of the business transactions}, making it less dependant on the supporting technology stack and, therefore, more portable.
%In fact, it is \textbf{only necessary to watch the throughput of the business transactions}, making it less dependant on the supporting technology stack and, therefore, more portable.
Another main advantage is the anomaly detection algorithm simplicity,  which makes it easier to train, to understand, and to tweak than other algorithms that need complex learning processes.
These factors make the overall methodology easier to use and more applicable in practice.


%Focusing on measurements of business transactions;
%Focusing on throughput instead of response time;
%Use  experimental results to calibrate the analytical model and to be able to answer the following questions:
%What are the tradeoffs between rate of attacks and rate of false positive
%Formulate an optimization problem using as cost function the rate of false positives and security intrusions detection time
%What would have been the impact of selecting different BA tuning parameters
%We show experiments to validate this methodology.
%Using TPCx-V
%Using performance degradation faultload



In summary, the paper's contributions are the following:

$(i)$ A novel \textbf{anomaly detection methodology for detection of performance degradation attacks} based on the bucket algorithm and monitoring of the throughput of business transactions (Section~\ref{sec:meth}).

$(ii)$ An \textbf{analytical model to parameterize anomaly detection mechanism}, which allows conducting principled parameterization. The model can be used to cope with the tradeoff between time to detect an attack and the rate of false alarms (Section~\ref{sec:ad_algo}).

$(iii)$ An \textbf{experimental assessment  of the methodology in practice} using a representative system and attacks. We established the feasibility of detecting attacks based on non-intrusive user-level performance metrics that are available in production environments (Sections~\ref{sec:expEnvl}-\ref{sec:results}).

$(iv)$ A \textbf{model-driven principled mechanism design} that allows revisiting the experimental results and conduct what-if analysis to assess different performance metrics of the considered anomaly detection algorithms as a function of the parameterization (Section~\ref{ssec:modelbasedinsights}). 



% NAO TEMOS NADA DISTO :-)
%\textbf{Measurement campaign and insights:} we conduct a large scale measurement campaign to determine the impact of  attacks on the performance of virtualized services. 
%The campaign is executed using the TPCx-V workload,
% and serves to illustrate the applicability of  the proposed anomaly detection methodology. % (Section~\ref{sec:expCamp}).
%,  profiled during a set of executions.
%We selected a set of resource exhaustion attacks to emulate the effects of anomalies affecting system performance. 
%The results show that our approach was able to successfully detect the anomalies, with a low number of false positives, and also spot possible residual effects on the system.  
%
% -- and we show the feasibiity of parameterizing through the proposed model-based approach.
%
%

% The proposed  approach is  non-intrusive --  most of the data needed to support the approach is commonly available in production environments 



% \color{red}\nuno{Longo. Volto no fim corrigir, quando tiver uma ideia.}



The remainder of the paper is organized as indicated in the summary of contributions above.  
Section~\ref{sec:related} covers related work, followed by our contributions in Sections~\ref{sec:meth}-\ref{sec:results}. 
Section~\ref{sec:threats} covers threats to validity and Section~\ref{conc} concludes.

\begin{comment}
Section~\ref{sec:meth} introduces the new methodology for anomaly detection in complex virtualized environments, followed by the considered anomaly detection mechanism and its analytical model in Section~\ref{sec:ad_algo}. % In Section ~\ref{sec:ad_algo} we present the introduced heuristic for anomaly detection.
Sections~\ref{sec:expEnvl}-\ref{sec:results} describe the target system and the supporting infrastructure to conduct our experiments, along  with our  experimental results. % and  empirical  experimental results.%  In Section ~\ref{sec:results} we present the analysis of the obtained results. 
The model-driven parameterization of the anomaly detection mechanism is presented in Section~\ref{ssec:modelbasedinsights}.

\end{comment}
  % contains our conclusions and suggestions for future research. 
% The Appendix contains the  performance analysis of the anomaly detection approach  and  the related optimization problem.

\color{black}

\section{Related Work} 
\label{sec:related}

% \toCG{\na{Sinto o bg/rw curto para um paper deste género. É apenas um feeling, ainda não li.}\\
% \cg{Vamos atacar os pontos mais criticos, fechando a maior parte, ataco aqui. Entretanto vou pedir ao daniel para adicionar algo da parte analitica aqui.}}

%\cg{Should some of this ''Related work's´´ be spread throughout the work instead of being on this section ?}

%\toCG{Virtualization issues}
In this section, we revise  related  literature indicating how  the current work relates to  prior art.

%our research in the following domains: 

% (1) security issues related to cloud multi-tenancy, (2) IDS implementation using anomaly detection, (3)  anomaly detection using sequential hypothesis testing and (4) anomaly detection approaches using performance signatures.

%, and (5) metrics to benchmark security	vulnerability	detection	tools.

\subsection{Security issues related to cloud multi-tenancy} 

Multi-tenancy with isolation among tenants is the standard model  in cloud-computing  environments. 
However, regardless of the  hardware isolation mechanisms used, there have been many recently reported security intrusions  across these isolation barriers~\cite{Hunt2019}.  % An attacker co-located at the same physical host as the victim can create a security threat  by using a malicious virtual machine that can cause side-channels attacks, or even system resource exhaustion  causing a \gls{dos}~\cite{Gruschka2010,krishna2017virtualization}.
%
%
In~\cite{krishna2017virtualization, Gruschka2010},  the authors discuss security issues related to running the hypervisor in cloud environments. For example, a  malicious virtual machine running over the hypervisor could attempt to break the hardware isolation 
barrier, violate privacy rules or attempt to compromise the hypervisor, e.g., through a system resource exhaustion  causing a \gls{dos} attack. The papers also discuss  architecture features that would be needed to   mitigate these security vulnerabilities. In this paper, we focus on detecting anomalies in operational systems under the assumption that the aforementioned vulnerabilities cannot be fully prevented.   


 The tracking of system calls can be used to implement  Intrusion Detection Systems for virtualized environments~\cite{Alarifi2012}.  The idea consists of  watching, during execution,  for anomalous system call sequences in the user programs.   The assessment used a Linux KVM  virtual machine to collect the system calls from user programs. Results show a trade-off between detection result and time efficiency when comparing different system call sequence lengths.  Nonetheless, benchmarking the performance of IDS tools  is a challenging problem~\cite{antunes_metrics_2015}, motivating simpler and interpretable detection methods. Our work is complementary to~\cite{Alarifi2012}, as we indicate that IDS systems can benefit from  anomaly detection  approaches which are less intrusive than those reported in~\cite{Alarifi2012}, relying on~\cite{Alarifi2012} only on specific scenarios. 



% A key element of IDS systems are the  metrics monitored in real time.  In~\cite{antunes_metrics_2015}, the authors discuss	which metrics shall be used to benchmark security	vulnerability	detection	tools.	The	presented analysis showed that the	best metric	alternative	
% depends	on	the	usage	scenario.



\subsection{ Anomaly detection for cybersecurity} 

% :   hypothesis tests and performance signatures }

An approach for anomaly detection consists in running sequential hypothesis tests~\cite{ho2011fast,jung2004fast}.
In~\cite{jung2004fast},  sequential hypothesis tests are used for  the detection of malicious port scanners. The authors have developed a link between the detection of malicious port scans and the theory of sequential hypothesis testing. They have also shown that port scanning can be modeled as a random walk.  The detection algorithm matches the random walk to one of two  stochastic processes, which correspond to malicious remote hosts or to authorized remote hosts.  The approach considered in this paper is similar in spirit to that considered in~\cite{ho2011fast,jung2004fast}, as our analytical results are derived from a  birth-death Markov chain. Such Markov chain can be interpreted as a random walk  through buckets which fill as the system degrades, and empty as the system recovers (see Section~\ref{sec:analytmodel}).  


% The stochastic process classification is used to develop an anomaly detection algorithm, which was named TRW (Threshold Random Walk). The authors have shown that their anomaly detection algorithm only needs a small number of connection attempts   to detect malicious activity.
% The analysis of the anomaly detection algorithm stochastic behavior, allowed the authors to derive theoretical bounds on
% the probabilities of missed detection (false negatives) and false alarms (false positives).
%%compare to the \gls{ba} 
%%can we derive false negatives and false %% %% bounds positives using similar 

% \subsection{Anomaly detection  using performance signatures}


A number of previous works have considered anomaly detection approaches  using performance signatures~\cite{ Cherkasova2009, avritzer2010monitoring}. 
%
%\toCG{performance monitoring}
The work in~\cite{Cherkasova2009} introduces a framework that detects anomalous application behavior using regression-based models and application performance signatures. This method uses the concept of profiling  system resources, such as  CPU demand. Then,~\cite{avritzer2010monitoring} builds on top of~\cite{Cherkasova2009} and proposes an anomaly detection approach based on performance signatures based on CPU, I/O, memory and network usage   for the detection of security intrusions. The approach has been shown to  outperform, in some cases,  intrusion detection systems based on security intrusion history~\cite{milenkoski2015evaluating}.

The performance of signature-based intrusion detection systems rely on  intrusion detection algorithms that account for workload variability  to avoid a high rate of false positive alerts.  An example of such workload-sensitive algorithms is the \gls{ba}  that was introduced in~\cite{Avritzer2005} and is presented in detail in Section~\ref{sec:ad_algo}.
%presented in Section~\ref{sec:framework} and
% introduced in~\cite{Avritzer2005}.
%In addition, there is a need to detect baseline profile changes. 
Anomaly detection using the \gls{ba}  inspects the last sample of response time and compares it against the calibrated mean and standard deviation of response time. Then, it relies on the central limit theorem~\cite{AvritzerBGTW06} to assess if the last samples of response time comply with normal behavior or represent an anomaly. 
In Section~\ref{sec:ad_algo}  
we revisit the \gls{ba} mechanism, and present an analytical model that is instrumental to parameterize the \gls{ba} from experimental data.

% for anomaly detection in complex virtualized environments, and we revisit the 
% revisit the \gls{ba} mechanism, and.

%\toCG{metrics to detect anomalies}
% {\bf Metrics to benchmark security	vulnerability	detection	tools }


\setcounter{figure}{1} % aldrabice por causa das figuras

\begin{figure*}[!hb]
    \centering
    \vspace{-5pt}
    \includegraphics[width=0.9\linewidth]{./img/meth.pdf}
    \vspace{-5pt}
    \caption{Detailed representation of the methodology. We can observe three distinct sets of runs of the system: \textbf{E}xploratory, \textbf{P}rofile, and \textbf{V}alidation}
    \label{fig:meth}
\end{figure*}

    
    \section{Attack Detection Methodology} 
    \label{sec:meth}
    
This section describes the proposed attack detection approach, which has the goal of helping the users to successfully apply our anomaly detection algorithm into the life cycle of their systems. An essential aspect of an anomaly detection approach is to be able to cope with changes in the operational profile, as the monitored systems commonly have different loads and demands over time. 
Our methodology follows a cyclic approach and foresees additional iterations to accommodate each new operational profile.  
    \figurename~\ref{fig:meth_lc} depicts the high-level application of the methodology.
    
    \setcounter{figure}{0} % aldrabice por causa das figuras
    
    \begin{figure}[ht]
        \centering
        \includegraphics[width=\linewidth]{./img/meth_lc.pdf}
        \caption{Overview of the methodology application life cycle.}
        \label{fig:meth_lc}
        %\vspace{-5pt}
    \end{figure}
    
    \setcounter{figure}{2} % aldrabice por causa das figuras
    
    
    As we can observe, the methodology consists of three main phases: 
    \textbf{(A) exploratory analysis}, which allows determining the most effective way to monitor the system based on its characteristics; 
    \textbf{(B) profiling}, which evaluates the system on its expected regular operational profile(s)~\cite{Musa1993} to extract information about the habitual behavior and its performance;
    and \textbf{(C) Operation}, in which the system executes for its intended purposes, and we use all data and knowledge from the previous phases and report deviations, identifying them as anomalies or attacks. 
    
    A new iteration is needed if changes are detected: 
    $i)$ in the system, demanding a new complete iteration to see if there are relevant aspects to add to the monitoring surface,
    $ii)$ in the operational profile, requiring to repeat the profiling. This does not mean that the previous parameters are obsolete, it could represent a profile change that can be expected within some periodicity (e.g. holiday/promotion seasons). 
    
    The phases of methodology are detailed in  \figurename~\ref{fig:meth}, and explained in the ensuing sections.
    
    
    %An application of this method leads to a monitoring cycle that,  during the daily system operation ($C_{1}$), allows the user to detect attacks ($C_{2}$) by getting alerts ($C_{3}$) and take action ($C_{4}$) to establish the regular operation. 
    %Also, the methodology can be integrated into the system's life cycle and adapted to routinely incorporate the changes that occur in the system's operational profile. 
    
    
    
    
    \subsection{Exploratory analysis phase}
    
    This phase has the objective of determining the monitoring surface used to monitor the system's performance.  
    To achieve that goal, the user needs to follow three main steps:  
    
    $A.1)$ \emph{Analysis:} evaluate the system's internal aspects like its architecture, components, operations and resources that are available for monitoring to define how to characterize the system performance
     
    $A.2)$ \emph{Exploration:} the tacit knowledge of the system is essential, and a set of executions of the system (\textbf{E} on \figurename~\ref{fig:meth}) is prescribed for exploratory analysis. 
    During those executions,  all monitored data should be collected and analyzed  to understand the metrics that effectively translate into useful measurements;
    
    $A.3)$  \emph{Definition:} use previous steps to determine the \textbf{monitoring surface}. The monitoring surface analysis is the effort of joining the tacit knowledge and internal aspects to define which components and metrics to use in the following phases. 
    
    
    \subsection{Profiling phase}
    
    %\nuno{WiP: evaluate the environment under execution on its regular operational profile (a quantitative characterization of how a system will be used~\cite{Musa1993}) to extract information about the expected behavior and the optimal way of assessing the performance of the system}
    
    %  regular operational profile(s)
    
    This phase has the objective of evaluating the environment during the execution of its expected regular operational profiles~\cite{Musa1993}, in order to establish the statistical parameters that represent those profiles. 
    The following procedures are needed: 
    
    $B.1)$ \emph{Golden runs definition:} the system is exercised under usual operational conditions, i.e., without any fault/attack to collect the available data using the monitor surface. 
    These system's executions are called \textbf{golden runs} and are the primary reference for the system's normal behavior.  
    We split them into two independent sets: one \textbf{P}rofile set used to compute the baseline metrics, and the second set used to \textbf{V}alidate the performance parameterization.
    
     
    $B.2)$ \emph{Baseline metrics extraction:} the computation of the baseline metrics is conducted extracting statistical data from the metrics defined over the monitoring surface. 
    Those extractions should be made for each subsystem, metric, operation and resource, and operational profile. 
    
    % The computation of the baseline metrics is defined accordingly with the performance monitoring algorithm used.  Those metrics should be set for each subsystem, metric, transaction, and operational profile.
    
    % Once the baseline metrics are established, we are ready to calibrate the performance model using the empirical data generated. We run several experiments using the Golden Runs data and the detection algorithm with different configurations. The performance model determines which parameters are best suitable for the tests.  We, then, account for the number of alerts that a given setting will cause.  Since we are assessing experimental runs under no attack conditions, we can define the algorithm tolerance for the number of false positives accordingly with the user's threshold goal.  The performance model will assist in minimizing the false positive rate. The calibrated performance model is the algorithm parameterization that is best suitable for the system-specific detection goals.
    
    % The final step is the baseline validation to check the validity of the determined parameters. We run the detection algorithm with the Golden Runs from the \textbf{V} group and check if the number of alerts (false positives) is in the defined experiment criteria.  If this is not the case, we can go back to the recalibrate the performance model until the requirements are fulfilled.
    
    
    $B.3)$ \emph{Performance model calibration:} apply the empirical data to determine the optimal values that minimize the false positives (FP) alerts. 
    The performance model determines which parameters are best suitable for the tests.  
    Then, we account for the number of alerts that a given setting will cause.  
    As we are assessing experimental runs under no attack conditions, we can define the algorithm tolerance for the number of FPs according to the user's preference.
    The performance model will assist in minimizing the FP rate. 
     
    $B.4)$ \emph{Baseline validation:} check the validity of the determined parameters. Apply the detection algorithm using the Golden Runs from the \textbf{V} group and check if the number of alerts (FP) is in the defined experiment criteria.  
    
    $B.5)$ \emph{Parameterization adjustment:}  during the baseline validation, if the alert rate does not meet the defined objective, we can go back and recalibrate the performance model until the requirements are met.
    
    
    
    \subsection{Operation phase}
    \label{sec:met_op}
    
    % \nuno{wip: Finally, on the Operation step, we use all data and knowledge from the previous components to search for anomalies or attacks during the system operation. }
    
    At this point, the anomaly detection algorithm is fully configured to monitor the system in production and detect security attacks that cause performance degradation. 
    Thus, in this phase, we take advantage of all the data and knowledge from the previous components to search for anomalies or attacks during the system operation.
    We need to:
    
    $C.1)$ \emph{Define a criterion:} that determines an alert condition in a concise manner. For instance, every alarm in any transaction or only alerts in critical subsystems?
    
    $C.2)$ \emph{Monitor the operation:} integrate the detection algorithm into the daily activity by continually watching  the monitoring surface using the detection algorithm with the optimal parameters
    
    
    
    


\section{Anomaly Detection Mechanism and Model} 
\label{sec:ad_algo}

In this section we describe the anomaly detection mechanism used in the proposed methodology and also the principled analytical model used. 

\subsection{Anomaly detection mechanism} 

%\toCG{ainda fala muito de response time}

The algorithm for anomaly detection heuristic based on performance degradation works by continuously  estimating  the mean response time, $\overline{x}$, and maintaining 
$B+1$ buckets of depth $D$ each, which contain  the  history of the most recent response times, as shown in \figurename~\ref{intrusion}. %The R notation is used to represent the point estimate of system response time.  
$P$ is a pointer to the
current bucket and $d$ is the number of recent response
time samples stored in the current bucket. 

Let $\mu$ be the baseline average response
time, and  $\sigma$ be the baseline standard deviation. Both $\mu$ and $\sigma$ can be  
derived from the execution of  the controlled  experiments (\textbf{golden runs}). The pointer $P$ to the current bucket is used to determine the current estimate of the average response time, which is given by  $\overline{x} = \mu + P  \sigma$. Once the current bucket overflows (resp., underflows), the algorithm estimate of the current average response time is shifted upward (resp., downward) by one standard deviation.  When all buckets overflow a performace degradation is detected and 
when all buckets underflow the system has recovered from a transient performance degradation. 

The performance degradation detection algorithm, that we will refer hereinafter as just Bucket Algorithm (\gls{ba}), is given as follows:

%\begin{enumerate}
\emph{Initialization:} $\{P\leftarrow 0; d\leftarrow 0 \}$, with all buckets empty.
 
\emph{Main loop:} for each sample $\hat{x}$ of response time, execute the steps below.
    
\begin{enumerate}
\item  if $P > B$, all buckets overflow, trigger performance degradation alarm;
\item if $\hat{x} > (\mu + P \sigma)$ then $\{ d \leftarrow d + 1 \}$,  response time larger than reference value, add token to the current bucket;
\item else do $\{ d \leftarrow d - 1\}$,  response time smaller   or equal than reference value, remove token from the current bucket;
\item if $(d > D)$ then do $\{ d \leftarrow 0; P \leftarrow P+1 \}$, current bucket overflow, go to next bucket;
\item if $\big((d < 0)$ and $(P >0)\big)$ then
do $\{ d \leftarrow D; P\leftarrow P-1\}$,  current bucket underflow,  go to previous bucket;
\item  if $\big((d < 0)$ and  $(P == 0)\big)$ then
do $\{d \leftarrow  0\}$ all buckets empty, system recovered from transient performance degradation.
\end{enumerate}
% \end{enumerate}

\begin{figure}
    \includegraphics[width=1\linewidth]{bucketsgraffle} \vspace{-0.2in}
    \caption{System of buckets diagram representing the dynamics of the detection algorithm. %, showing $B$ buckets of depth $D$ each. $P$ is the pointer to the current bucket and $d$ is the number of recent response times stored in bucket $P$.  Note that a buffer underflow indicates recovery from transient performance degradation, while the overflow of the last bucket triggers a security alarm.
    $D$ and $B$ must be properly parameterized for each operation}
    \label{intrusion}
    \vspace{-0.1in}
\end{figure}


The performance degradation detection algorithm can be tuned by varying the bucket depth, $D$, and the number of buckets, $B$.  The larger the product $D\times B$  the longer it takes  for the algorithm to detect the performance degradation. 
%However, shorter times of $D\times B$, would lead to a larger fraction of false positives. 
The statistical analysis  of the behavior of this family of \glsplural{ba} has been described on~\cite{AvritzerBGTW06}.


\subsection{Analytical model motivation and goals}



%\subsubsection{Motivation}

Sequential probability ratio test~\cite{jung2004fast} and the bucket algorithm~\cite{AvritzerBGTW06} are used to detect attacks in networks.  
Their analysis involves a random walk birth-death process.  
In the bucket algorithm, for instance, in the initial state all buckets are empty, and in the final state all buckets are full.  
Understanding the mean time to reach the final state, one can tune the number of buckets and the depth of each bucket in a principled way. 
%
%In this appendix, we present some preliminary ideas on the principled tuning of the bucket algorithm.  We envision that those preliminary ideas can be combined with recent advances in the study of birth-death processes (e.g.,~\cite{jouini2008moments}) to yield more refined results.
%
Simple algorithms to detect attacks, such as the bucket algorithm, can be tuned using first principles.


%\subsubsection{Goals}


%How does the depth of the bucket impact the probability of false positives?  
The larger the depth of the bucket, the lower the false positive probability, but the longer it takes for a true positive to be identified.
To simplify the analysis, we \textbf{work under the assumption} that attacks will change the response time distribution, and will always be detected.
However, the number of samples to detect the attack may vary depending on the depth of the bucket.
Our \textbf{second key simplifying assumption is} that the number of samples to detect the attack is much smaller than the number of samples collected before getting a false positive (which should be always the case in practice: the time until a false positive should be much longer on average than the time until a true positive).  

Then, we aim at answering the following question: what is the smallest bucket depth to produce a false positive probability bounded by a given threshold?

\subsection{Analytical model}
\label{sec:analytmodel}

Next, we introduce a 
discrete time birth-death Markov chain (DTMC) to characterize the behavior of the \gls{ba}. State $(b,d)$ of the Markov chain corresponds to the setup wherein there are $d$ balls in bucket $b$, and $D$ balls in buckets $b-1, \ldots, 1$.


Each  transition of the DTMC corresponds to the collection of a new sample. 
Such sample   causes the system to transition from state $(b,d)$ to one of its two neighboring  states. 
Let  $p_i$  be the probability that the number of balls at bucket $i$ increases after a new sample is collected.  
Then, $p_i=\mathbb{P}(\hat{x}  > \overline{x} + (i-1)\sigma),$ for  $ 1 \leq i \leq B$. 
The entries of the transition probability matrix are readily obtained from \figurename~\ref{fig:dtmc}, with the explicit expression of the transition probability matrix is presented in~\cite{techreport}.


\begin{figure}[ht]
    \centering
    \includegraphics[width=1\columnwidth]{newbucketdiagram.pdf}
    \caption{Discrete time Markov chain characterizing the behavior of the \gls{ba}.  Each transition corresponds to the collection of a new sample.}
    \label{fig:dtmc}
\end{figure}



  %given as follows:

\begin{comment}
  
  \begin{align}
     & p_{(k,d),(\tilde{k},\tilde{d})}= \\
      &\left\{
      \begin{array}{lll}
      P(\hat{x}  > \overline{x} + k\sigma), & \textrm{if } & (d < D, \tilde{d} = d+1,  k=\tilde{k}) \textrm{ or }   \\
             & &( d = D, \tilde{d} = 1,  k-1=\tilde{k} )  \textrm{ or } \\           &  & (d = D, k = K,      \tilde{k} = \textrm{absorbing})   \\
              P(\hat{x}  \leq \overline{x} + k\sigma), & \textrm{if } & (d > 1, \tilde{d} = d-1,  k=\tilde{k}) \textrm{ or }   \\
             & &( d = 1, \tilde{d} = D,  k+1=\tilde{k} )  \textrm{ or } \\           &  & (d = \tilde{d}= 0, k =\tilde{k}= 1),   \\
             0, & \multicolumn{2}{l}{\textrm{otherwise.}}   
      \end{array}\right.
 \nonumber \end{align}

\end{comment}
 
Once the terminal absorbing state  is reached  an alarm is triggered. The DTMC is illustrated for the case $B=2$ in \figurename~\ref{fig:dtmc}. 
The number of samples collected until absorption  accounts for a tradeoff between the mean time until $(a)$ a  false alarm, in the absence of attacks, and $(b)$ detection, in the presence of an attack.  Larger values of bucket depth  $D$ favor the reduction of the former but  increase the latter. 
 
Let $A_B(p_1,p_2,D)$ be the mean time until absorption, measured in number of collected samples, accounting for $B$ buckets of depth $D$ each. 
We derived a closed-form~\cite{techreport} expression for the time until absorption, which  is instrumental to handle that tradeoff.
In particular, for $B=2$, the resulting expression is given by
%
%Let $A_2$ be the time to absorption with $K=2$ buckets.   $A_2$ can be expressed as a function of $p_1$, $p_2$ and $D$,
\begin{align}
A_2(p_1,p_2, D)  %V_{D+1,1,0} + V_{D,2,1} \\
&= A^{(1)}_2(p_1,p_2, D)  + A^{(2)}_2(p_1,p_2, D) \label{eq:a2p1p2d}
\end{align}
where $A^{(i)}_B$ is the mean time to fill the $i$-th out of $B$ buckets,
\begin{align}
A^{(1)}_2 &=   { \Delta_1} \left(\delta_1- D\right) \\
A^{(2)}_2 %&=  \left( \frac{1+\rho_2}{1-\rho_2} + U_{0,2} \right)  \left(\frac{1-\rho_2^{-D}}{1-\rho_2^{-1}} \right) - D \frac{1+\rho_2}{1-\rho_2}   \\
% &=  \left( \Delta_2 + \Delta_1\frac{1-\rho_1^{D+1}}{\rho_1^{D+1}}\right)  \left(\frac{1-\rho_2^{-D}}{\rho_2-1} \right) - D \Delta_2 \\
&=  \Delta_2\left( \delta_2
-D\right) + \Delta_1\left(\frac{1-\rho_1^{D+1}}{\rho_1^{D+1}}\right)  \delta_2
\end{align}
%\begin{align}
%U_{0,2} 
%   &= \frac{1}{1-p_2} \left(1 + p_2  (\rho_1+1)\frac{\rho_1^{-D-1}-1}{1-\rho_1} \right) % \\
    % &=\frac{1+\rho_1}{\rho_1} \frac{1-\rho_1^{-n}}{1-\rho_1^{-1}} + \rho_1^{-n} ({1+\rho_1^{-1})}  
%\end{align}
and
\begin{equation}
    \rho_i = \frac{1}{p_i} -1, \qquad \Delta_i=\frac{1+\rho_i}{1-\rho_i}, \qquad \delta_i = \frac{1-\rho_i^{-D}}{\rho_i-1}.  
\end{equation}


% In what follows, we numerically illustrate the behavior of the quantities of interest and the subsumed tradeoff.

% \toCG{Notation Table ? \nuno{sera necessario?} \cg{Sugestão do daniel, disse muito comum, mas acho que podemos passar, só checar a consistência.} }

% \toCG{Check consistency over the paper K in the modeling would be the B in the empirical study \nuno{ja esta? ja nao acho K} \cg{Fazendo o double check! Removo o comentario em breve}}



\subsection{Parameterization of the anomaly detection mechanism:  a model-driven optimization approach}
\label{sec:param_ad}

\subsubsection{Why model-driven parameterization?}
 To compare different configurations of the \gls{ba} , we face the problem that the increase of $B$ or $D$ changes the detection sensitivity and time to alert.  

 To illustrate this phenomena, let us simplify the problem and consider that the system's transactions happens in a fixed interval time $t$. 
Assuming a critical workload, where all samples $\hat{x}$ (transactions) evaluated are always greater than the $(\mu + P \sigma)$, the minimum amount of time to detect any anomaly has a length of $BDt$. 
 For that reason, the number of maximum alerts within any time-specific $l$ is determined by $\frac{l}{BDt}$. That way, for another distinct configuration, if $B$ or $D$ increases, the number of possible alerts will decrease. 


 For that reason, the consideration of what defines a detection or its absence should be defined accordingly with the application and system. 



\subsubsection{Hypothesis testing}

The system administrator continuously considers two alternative hypothesis:  $(i)$ null hypothesis $H_0$ corresponding to a situation where there is no attack taking place
and $(ii)$ alternative hypothesis $H_1$ meaning that the system is under attack. Then, the key quantities of interest can be defined as a function of $H_0$ and $H_1$.

\begin{definition}
The  mean time until a false alarm under $H_0$ is denoted by $A_B$.  It is given by the mean time to  reach the absorbing state of the Markov chain characterizing the bucket algorithm.
\end{definition}



\begin{definition}
A lower bound on the  time until a true positive  under $H_1$  is denoted by $L$.  Assuming all buckets are initially empty, we let $
    L = BD$.
\end{definition}

\begin{definition}
The probability of false alarm is the probability that an alarm is triggered outside an attack,
$  f = \mathbb{P}(R < T), $ 
where $R$ is a random variable with mean $A_B$ characterizing the time until an alarm is triggered,  and  $T$ is  a random variable with mean $1/\alpha$ characterizing the time until an attack occurs.
\end{definition}


In this paper, except otherwise noted we assume that $f$ depends on $R$ and $T$ only through their means, i.e., $f = f(A_B, \alpha^{-1})$.



\begin{definition} \label{def:cost}
The expected cost of a given system parameterization is a weighted sum of the probability of false positives, computed under $H_0$,  and a lower bound of the time until detecting an attack, computed under $H_1$,
 \begin{equation}
     C(\bm{p}, w, D, B, \alpha)  =  B D +  w f(A_B, \alpha^{-1})  \label{eq:cost1}
 \end{equation}
\end{definition}



\subsubsection{Modeling the probability of false alarms} 
We assume that attacks arrive according to a Poisson process with rate $\alpha$. 
Let $f$ be the probability of a false alarm.  We consider two distinct models to determine the probability of false alarm as a function of $A_2$ and $\alpha$. The deterministic  (resp., exponential) model  presumes that  the number of samples taken until a false alarm can be well  approximated by  a deterministic (resp., exponential) distribution with mean  $A_2$.  
 Then,
\begin{equation}
    f = \varphi(A_2 \alpha) 
\end{equation}
\begin{comment}
\begin{equation}
    f = \varphi(A_2 \alpha)  e^{- A_2 \alpha} \label{eq:fexp1}
\end{equation}
and
\begin{align}
    f = \frac{1/A_2}{\alpha + 1/A_2}  =  \left( 1+{A_2}{\alpha} \right)^{-1} \label{eq:fexp2}
\end{align}
\end{comment}
where $\varphi(x) = e^{-x}$ and $\varphi=1/(1+x)$
under the deterministic and exponential models, respectively.


\subsubsection{Optimization problem formulation} \label{sec:optimization}

Given a target false positive probability, denoted by $F$, the system administrator goal is to  determine the optimal number of buckets and bucket  depth so as to 
minimize the lower bound on number of samples to detect and attack, $L$, while still meeting the target false positive probability. 
\begin{align}
&{\mbox{\sc  Problem with Hard Constraints:}}\quad  \nonumber \\
&    \min \quad L=BD \\ \label{eq:hard}
 &   \textrm{subject to} \quad f(B,D) \leq F  
\end{align}
In what follows, we assume that $B$ is fixed and given.  Then, as $f$ is strictly decreasing with respect to $D$, the constraint above will be always active and the problem translates into finding the minimum value of $D$ satisfying the constraint.  The problem above is similar in spirit to a Neyman-Pearson hypothesis test, for which similar considerations apply, i.e., the optimal parameterization of the test is the one that satisfies a constraint on the false positive probability.  

Alternatively, the problem above can be formulated through the corresponding Lagrangian, 
\begin{align}
&{\mbox{\sc  Problem with Soft Constraints:}}\quad \nonumber  \\
& \min     \mathcal{L}(D) = B D + w (f(B,D)- F)  \label{eq:lag} 
\end{align}
where $w$ is the Lagrange multiplier.  The Lagrangian naturally leads to an alternative formulation of the problem, wherein  the hard constraint in~\eqref{eq:hard} is replaced by a soft constraint corresponding to the penalty term $f(B,D)- F $ present in the cost Lagrangian. The Lagrangian is a cost function, motivating Definition~\ref{def:cost}. Note that as $wF$ is a constant, minimizing~\eqref{eq:lag} is equivalent to minimizing~\eqref{eq:cost1}.

\begin{comment}
Note that whereas the {\mbox{\sc  Problem with Hard Constraints}} is defined as a function of the target false alarm probability $F$, the {\mbox{\sc  Problem with Soft Constraints}}   is defined as  a function of the weight $w$.  Although there is a mapping between the two problems, the target false alarm probability may be easier to interpret as it has a concrete physical interpretation as opposed to $w$, which is a Lagrange multiplier.  Nonetheless, the cost function defined by $w$ allows to visually determine the value of $D$ that minimizes cost. For this reason, the two formulations may be complementary, as indicated in the upcoming section through a numerical example parameterized using data from our controlled experiments. 

\end{comment}

\section{Experimental Validation} 
\label{sec:expEnvl}

To demonstrate and validate the methodology described in Section~\ref{sec:meth}, we defined an experimental study that uses the \gls{tpcxv}, which is representative of complex systems that take advantage of virtualization to support businesses, as presented in Section~\ref{ssec:sut}.
The operational phase is emulated through a series of runs of the benchmark in which we inject a set of faults that emulate the effects of attacks that affect system performance, as explained in Section~\ref{ssec:faults}. 
We go over all the phases  to apply the proposed methodology, describing the main considerations and the key data obtained in each step, including the performed exploratory analysis in Section~\ref{ssec:sut-exploratory},
the profiling phase in Section~\ref{ssec:sut-profiling}, the operational phase in Section~\ref{ssec:sut-operational}, and the model calibration in Section~\ref{ssec:modelbasedinsights}.



\subsection{System Under Test} 
\label{ssec:sut}

The typical virtualization environment that is representative of a real-world scenario of cloud computing providers, can be quite complex and have many properties that are difficult to emulate in a practical testbed.  
In this work, we are interested in a compromised multi-tenant cloud computing infrastructure, which is composed by several users sharing this infrastructure, one of which trying to exploit the vulnerabilities present on the underlying hypervisor.    



The \gls{tpcxv} is a public available, end-to-end benchmark for data-centric workload on virtual servers. The benchmark kit provides the specification,  implementation, and tools to audit and run the benchmark. Details can be found in~\cite{tpcv2013, tpcv2015}.
It models many features commonly present in cloud computing environments such as multiple \glspl{vm} running at different load demand levels, and significant fluctuations in the load level of each \gls{vm}~\cite{tpcv2013}.  
We use the workload and software provided by the \gls{tpcxv}\cite{tpcv2015} to emulate a context closely related to a real-world scenario of brokerage firms that must manage customer accounts, execute customer trade orders, and be responsible for the interactions of customers with financial markets.

\figurename~\ref{fig:tpc-arch} shows the transaction flow. 
The virtual client emulator (vce), interacts with the different brokerage firms (distinct groups), which in turn communicates with the virtual market emulator (vme). 
%may be viewed as a Data Center in a Box'' as it 
\gls{tpcxv} uses virtualization technology to co-locate database tiers and application-management tiers on logically distinct \glspl{vm} within a single computer system.

%\figurename~\ref{fig:businesmodel} illustrates the different entities modeled by the \gls{tpcxv} and the related transactions among them. 

% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.9\linewidth]{./img/transFlow_v2.pdf}
% \caption{ \scriptsize Business Model Transaction Flow}
% \label{fig:businesmodel}
% \end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=.9\linewidth]{./img/tpc-arch.png}
    \caption{TPCx-V components and transactions flow (from~\cite{TPCx-V_spec}). In this work, each group is treated as distinct subsystem. } 
    \label{fig:tpc-arch}
\end{figure}

The goal of \gls{tpcxv} is to measure how a virtualized server runs database workloads, using them to measure the performance of virtualized platforms, specifically the hypervisor, the server hardware, storage, and networking. The minimal deployment of the \gls{tpcxv} will have four groups, each with three \glspl{vm}, representing different subsystems that contribute differently for the overall load during the {\bf{}}  { \bf{ \texttt{10} distinct load phases} of \texttt{12} minutes}  that exist during a typical run. 
The different components of \gls{tpcxv} are architecturally distributed as depicted in \figurename~\ref{fig:tpc-arch}

The \gls{tpcxv} workload is made up of \textbf{\texttt{12} types of transactions} with different characteristics that are submitted for processing at multiple databases (market, customer, and broker) following a specified mix of transactions for different phases. 
Transactions are used to simulate the stock trade process, and when a trade finishes, a transaction name \textit{Trade-Result} is issued. 
The primary performance metric for the benchmark works as a business throughput and is known as \texttt{tpsV}, and portrays the number of completed \textit{Trade-Result} per second.


%Additionally to the specification, the benchmark kit comes with a set of software components with its implementation and tools to audit and run the benchmark. 
%Discussion about experimental performance metrics, design considerations,  tunning deployments, and others practicals considerations of the \gls{tpcxv} are present in~\cite{tpcv2013, tpcv2015}.  


Our \textit{experimental setup} is a deployment of the \gls{tpcxv} over two physical servers. The first, a Dell PowerEdge R710 with 24 Cores, 96 GB RAM, and 12 TB disk, managed by a Xen hypervisor (4.4.1), has a privileged domain (dom0), and 17 virtual machines with different configurations, a set dedicated to the \gls{tpcxv} and other that will represent our compromised tenants. Another server, with 2 Core, 8GB RAM and 1 TB disk, with the same hypervisor, host the \gls{vm} driver component into a different host as prescribed on the \gls{tpcxv} specification. The details of each \gls{vm} is described in \tableautorefname~\ref{tab:vms_spec}.

As we can see in the \tableautorefname~\ref{tab:vms_spec}, the resources specifications varies for each group (tpc-g\textit{n} refers for a \gls{vm} for group \textit{n}) and it was defined following the recommendations on~\cite{TPCx-V_spec}.  Since a group is a set o three \gls{vm}, our malicious user will have access to the same amount of \glspl{vm}. 


\begin{table}[t]
\centering
\caption{ \scriptsize  \glspl{vm} name, memory and the number of virtual CPUs. The tpc-driver is supported on a different physical host}
\label{tab:vms_spec}
\vspace{-0.05in}
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{ccc||ccc||ccc}
\toprule

\textbf{\gls{vm} } & \textbf{MB}  & \textbf{vCPU}   & \textbf{\gls{vm}} & \textbf{MB}  & \textbf{vCPU}  & \textbf{\gls{vm}} & \textbf{MB}  & \textbf{vCPU}     \\ \midrule
tpc-g1a         &   1024    & 1  & tpc-g2b2        &   6144    & 6  & tpc-g4b1        &   20400   & 2 \\
tpc-g1b1        &   8192    & 2  & tpc-g3a         &   1024    & 1  & tpc-g4b2        &   10240   & 8 \\
tpc-g1b2        &   4096    & 4  & tpc-g3b1        &   16384   & 2  & tenant A        &   1532    & 2 \\
tpc-g2a         &   1024    & 1  & tpc-g3b2        &   8192    & 8  & tenant B        &   1532    & 2 \\
tpc-g2b1        &   12288   & 2  & tpc-g4a         &   1024    & 2  & tenant C        &   1532    & 2 \\ \midrule
dom0            &   1962    & 4  & tpc-driver\footnotemark[1]      &   1882    & 2 & & &\\ 
\bottomrule
\end{tabular}
%\vspace{-0.15in}
\end{table}

We developed tools to trigger all tests, start benchmark components, report any problem during the test, and manage all the interactions between the environment, benchmark, and tests.  
Each \textbf{single experiment lasts roughly 4 hours} that correspond to the 2h demanded as minimum by the benchmark specification, and another 2h to restore the system.
These tools restore the environment to the same initial state to ensure the reproducibility across different experiment runs. 
It does this action basically by rebooting the servers and recovering the system and databases (restoring all virtual disks).







% \begin{table}[ht]
% \small
% \centering
% \caption{ \scriptsize \glspl{vm} resource specifications}
% \label{tab:vms_spec}
% \begin{tabular}{@{}ccc@{}}
% \toprule
% \textbf{\gls{vm} name} & \textbf{Memory(MB)}  & \textbf{vCPU}      \\ \midrule
% dom0            &   1962    & 4 \\
% tpc-g1a         &   1024    & 1 \\
% tpc-g1b1        &   8192    & 2 \\
% tpc-g1b2        &   4096    & 4 \\
% tpc-g2a         &   1024    & 1 \\
% tpc-g2b1        &   12288   & 2 \\
% tpc-g2b2        &   6144    & 6 \\
% tpc-g3a         &   1024    & 1 \\
% tpc-g3b1        &   16384   & 2 \\
% tpc-g3b2        &   8192    & 8 \\
% tpc-g4a         &   1024    & 2 \\
% tpc-g4b1        &   20400   & 2 \\
% tpc-g4b2        &   10240   & 8 \\
% tenant A        &   1532    & 2 \\
% tenant B        &   1532    & 2 \\
% tenant C        &   1532    & 2 \\ \midrule
% tpc-driver\footnotemark[1]      &   1882    & 2 \\ \midrule
% \bottomrule
% \end{tabular}
% \end{table}
% \footnotetext[1]{Supported on a different physical host}






\subsection{Fault Model}
\label{ssec:faults}



The fault model used in our work explores one of the possibles attack models on cloud computing: the resource exhaustion pattern~\cite{Gruschka2010}.  In this kind of attack, the virtual guest can obtain more resource than allowed or even lead the system into a Denial-of-Service state. 
They can be divided into two main categories~\cite{Groza2011}: 
i) \textit{excessive use}, where there is no abnormal use, but the consumption of resources is significantly higher than the others; and 
ii) \textit{malicious use}, where the intentional abuse of the resources lead the system to a failure state.

Since the \gls{tpcxv} has a database workload, an attack that explores the primary resources used in these systems will surely have an impact on the performance and, consequently, the reference metric of the system.
To the best of our knowledge, we are unaware of a real exploit tailored for virtual environments that focus explicitly on the hypervisor and tries to exhaust the typical resources used on database services. 

To overcome the absence of a representative attack, we simulated a resource exhaustion behavior by using the Stress-NG software~\cite{stressng}, which was designed to ``exercise various physical subsystems of a computer as well as the various operating system kernel interfaces'' and can be parameterized to perform many IO and CPU operations in various forms. 
We defined three configurations to emulate our attack and test our system:  

 \textit{(H):}  A High-Intensity workload: during 300 seconds it starts eight processes to abuse the system IO;
 
 \textit{(L):} A Low-Intensity workload: during 300 seconds, we perform ten intervals of 15 seconds of IO-abuse and 15 with no workload.  The workload uses two IO stressors processes;
  
 \textit{(Ls):} Shorter Low-Intensity workload: the same as the (L) configuration but with only three intervals.
  






We defined the duration of the configuration based on proportional time of the \gls{tpcxv} run, roughly 4\% and 1\%. The configurations length are also less than the benchmark phase (\texttt{12} min, as explained in Section~\ref{ssec:sut}). The number of IO process was defined empirically, running different configuration and checking which one did not freeze the Guest-VM or was not too small to do not be considered abusive. We will reference those configurations as H, L, and Ls, respectively.

% \toNA{Think about the testing name : change the 6 and 4 for a more significant name : \toCG{maybe we can just name the test when it is on the peak performance and non-peak performace...  It will be P and nP ... PH \textit{P}L \textit{nP}Ls}}


Since the \gls{tpcxv} has different phases with diverse load demands (see Section~\ref{ssec:sut-operational}), we focused the attack on two distinct phases, on the \texttt{4th}, which is when \textbf{the group with more physical resources has a more significant contribution to the overall load}  and the \texttt{6th}, when \textbf{the reference metric achieves the highest rate}. 

Combining those two definitions, we have a total of \texttt{6} fault models, which we will refer to using the phase plus the configuration reference: \texttt{4H}, \texttt{4L}, \texttt{4Ls}, \texttt{6H}, \texttt{6L}, and \texttt{6Ls}.






\subsection{Exploratory Phase}
\label{ssec:sut-exploratory}

The first part was to understand the  \gls{tpcxv} architecture, and its specification to get some tacit knowledge about its deployment in our environment.  
In previous works~\cite{AvritzerBGTW06,avritzer2010monitoring},  the \gls{ba} was applied using response time as the anomaly detection metric. 
In this work, we are evaluating a complex system with different components and subsystems that aims to maximize its throughput. 
Hence, we decided to also use the system's throughput as the input metric for the \gls{ba}.   

Based on the response time data available from the \gls{tpcxv} results, we derived a throughput extraction process that aggregates the transactions by group, phase, transaction type, and  the operation completion time. 
Also, to accommodate a metric that is best when its value is short (contrary to the response time), we changed the algorithm to invert the logic. 
It will penalize the metric if its value is lower than the average plus a multiple of the standard deviation, i.e., $\hat{x} < (\mu + P \sigma)$.

The next step was to perform several exploratory runs, that allowed to conduct a characterization of every transaction and applied the \gls{ba} in all data collected to make a preliminary assessment. 
The analysis revealed that not all of the \gls{tpcxv}'s transactions are useful in reflecting the system's load. 
Additionally, the results from the response time evaluation showed an higher variability that leads to a higher number of false alarms.

Concluding the exploratory phase, we defined our monitoring surface as the throughput information of \texttt{9} (of the \texttt{12}) transactions from \gls{tpcxv}. 
That data will be evaluated distinctly for every subsystem (the \texttt{4} \gls{tpcxv}'s groups), resulting in \texttt{36} (\texttt{9x4}) bucket algorithms running, each with \texttt{10} distinct configurations, \texttt{1} for each distinct operation profile (the \texttt{10} \gls{tpcxv}'s phases). 


% After evaluating the algorithm using both metrics, we rapidly noticed that by using the throughput data, we have better results as \tableautorefname~\ref{tab:rtVsTput} shows.  Additionally, some results are different. For instance, in the run 595 (6H), we did not alert in the injection period using the RT, but it did report using the throughput database.

% \begin{table}[ht]
% \normalsize
% \centering
% \caption{Performance comparison for b=2 and d=15}
% \label{tab:rtVsTput}
% \begin{tabular}{cccc}
% \toprule
% & \textbf{TP} & \textbf{FP} & \textbf{Precision\footnotemark[1]} \\ \midrule
% Response Time & 182 & 522 & 25,85\% \\
% Throughput & 1874 & 38 & 98,01\% \\ 
% \bottomrule
% \end{tabular}
% \end{table}
% 
% \footnotetext[1]{For this precision account we simply counted the number of alerts inside and outside the attack period.}


\subsection{Profiling Phase}
\label{ssec:sut-profiling}

To profile the system, we executed 59 golden runs to generate data for the characterization of the system's baseline behavior (37 runs, {\it P set}) and also validation (22 runs, {\it V set}).  
For every transaction from the monitoring surface, we compute and store the average throughput for each subsystem in every operational profile.   
These values are the system's baseline metrics. 

To calibrate our performance model (Section~\ref{ssec:modelbasedinsights}), we need to account for the following metrics:  
\begin{enumerate}
    \item The probability of a false positive alarm as a function of bucket depth;
    \item The probability for each transition in the DTMC (\figurename~\ref{fig:dtmc});
    \item The mean time to first alarm during an attack.
\end{enumerate}

To compute those probabilities, we applied the \gls{ba} with different configurations over the {\it V set} runs data. 
These results are presented in Section~\ref{sec:results}.

For the validation process, we applied the \gls{ba} for every golden run, accounting for the number of alerts (false positives). 
The goal of this step is to check if using the parameters suggested by the model will not generate an unacceptable amount of false-positive alerts.
First, we execute the assessment with the same runs used to generate the baseline metrics ({\it B set}). 
Here we are not validating, only producing values to compare later with the validation results.  
Also, this step can use for consistency check and test for possible computational errors if the results show any abnormal number of alerts. 
Then we repeat the process using the validation runs ({\it V set}). 
The results of both sets are not significantly different, and thus we present only the validation values in~\tableautorefname~\ref{tab:basel_param}.

We can see in \tableautorefname~\ref{tab:basel_param} that using two buckets is more effective, as it shows a fair number of false-positive alerts. 
One bucket has too many alerts, and three is likely to be ineffective.

\begin{table}[ht]
%\small
\vspace{-0.1in}
\centering
\caption{\scriptsize  False positive alerts: total count and average ($\mu$) by run in validation}
\label{tab:basel_param}
\vspace{-0.05in}
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{cccc||cccc||cccc}
\toprule
\textbf{B} & \textbf{D} & \textbf{\# Alerts} & \boldmath$\mu$  
& \textbf{B} & \textbf{D} & \textbf{\# Alerts} &  \boldmath$\mu$ 
& \textbf{B} & \textbf{D} & \textbf{\# Alerts} & \boldmath$\mu$  \\\midrule

1 & 30 & 27373 & 1244,23 & 2 & 12 & 4 & 0,18 & 2 & 21 & 0 & 0,00 \\
2 & 6 & 185 & 8,41 & 2 & 15 & 0 & 0,00 & 3 & 10 & 0 & 0 \\
2 & 9 & 12 & 0,55 & 2 & 18 & 0 & 0,00 & & & & \\\bottomrule
\end{tabular}
\end{table}


Looking at the \tableautorefname~\ref{tab:basel_alert_txns}, we can see that for distinct transaction types, we have distinct sensitiveness for the same parameterization when applying the \gls{ba}.  These distinct sensitivities can suggest that different values for $D$ should be applied for different operations.

\begin{table}[ht]
%\small
\vspace{-0.1in}
\centering
\caption{\scriptsize  False positive alerts segmented by \gls{tpcxv}'s transactions }
\label{tab:basel_alert_txns}
\vspace{-0.05in}
\begin{tabular}{cc|ccccccccc}
\toprule
\multicolumn{2}{c|}{ \textbf{Transaction ID} } & 0 & 1 & 2 & 4 & 5 & 6 & 7 & 8 & 9 \\
\midrule
\multirow{3}{*}{ \textbf{D} } & 6 & 23 & 43 & 28 & 34 & 12 & 23 & 14 & 2 & 6 \\
& 9 & 0 & 1 & 4 & 6 & 1 & 0 & 0 & 0 & 0 \\
& 12 & 0 & 0 & 2 & 2 & 0 & 0 & 0 & 0 & 0 \\\bottomrule
\end{tabular}
\end{table}


When running the \gls{ba} in both golden runs sets, we obtain similar results. This similarity indicates that the profile derived from the baseline metrics generalizes for different runs.

After the previous analyses, we were able to apply the performance model in the experimental data. Section~\ref{ssec:modelbasedinsights}  details the complete process. The calibrated performance model suggests $D \in (12,15]$, and the number of alerts withing this range is acceptable. 




\subsection{Operational Phase}
\label{ssec:sut-operational}

%In this experimental campaign, we will adapt the methodology operation step to perform an empirical study of the \gls{ba} applicability.

As prescribed in Section~\ref{sec:met_op}, we have to define our alert criterion.  
We adopted distinct approaches to detect \textit{true positives} (TP) and \textit{false positives} (FP).  
A TP is when we detect {\bf at least one alert on the attack phase}. 
We only need one alert in any group for any transaction type. 
Complementarily, a \textit{False Negative} (FN) is when \textbf{no alert is raised} on the same phase.  
We consider an FP \textbf{every bucket overflow that happen in the no-attack phase}. 
In this case, two bucket overflows in distinct transactions, or even in the same, but in different groups, will account for two distinct FP. 
This approach is justified as in any detection system, a better tool is the one that is effective and minimizes the number of false positives. 

An alert on the post-attack phase can be an FP or either a residual effect caused by the faultload. 
For that reason, we cannot assert exactly anything about it, but we will discuss this further in Section~\ref{sec:re}.

At last, the \textit{true negative} (TN) is not necessary to be defined.  
The problem is that the \gls{ba}  is designed to detect a deviation from the regular operation continuously during its execution.  
To estimate the number of possible alerts during a specific period, based on a fixed detection window, does not make sense when comparing different workloads and configurations (see Section~\ref{sec:param_ad}).

During the testing campaign process, each of our test runs is composed of three phases, as depicted in \figurename~\ref{fig:testDesc}.  
In those periods defined, we will count the number of FP, TP, and FN as described early. 
Each alert on the post-attack phase will count as a {\it residual effect}.  
When executing the \gls{tpcxv} workload, we will run just one attack, as defined in Section~\ref{ssec:faults}. 
As showed in \tableautorefname~\ref{tab:runs}, we performed 21 runs for each fault injection type, while applying the \gls{ba} throughout the monitoring surface.

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{./img/test_desc_v2.pdf}
    \caption{Distinct phases and its alerts meaning during a test run.}
    \label{fig:testDesc}
\end{figure}

\begin{table}[ht]
    \vspace{-0.1in}
    %\small
    \centering
    \caption{Runs in Experimental Campaign}
    \label{tab:runs}
    \vspace{-0.05in}
    \begin{tabular}{c||cccccc||c}
    \toprule
    Test & 4H & 4L & 4Ls & 6H & 6L & 6Ls & Golden \\
    $N^{o}$ Runs & 21 & 21 & 21 & 21 & 21 & 21 & 59 \\\bottomrule
    \end{tabular}
\end{table}


After the test executions, we used the data collected to apply the \gls{ba} with different parameterizations to study the effectiveness of the method. 
An initial observation, based on the data presented in previous analysis and  \tableautorefname~\ref{tab:bd_variat}, is that the optimal number of buckets is two.
But which specific configuration is more effective in which failure mode are demonstrated in the next section.


\begin{table}[b]
    %\normalsize
    \centering
    \caption{\scriptsize Fraction of attack alerts over all alerts varying $B$ and $D$. We are accounting all alerts, not following the detection's criterion.}
    \label{tab:bd_variat}
    \vspace{-0.05in}
    \setlength\tabcolsep{3pt} % default value: 6pt
    \begin{tabular}{ccr|ccr|ccr|ccr}
    \toprule
    \textbf{B} & \textbf{D} & \textbf{\%} & 
    \textbf{B} & \textbf{D} & \textbf{\%} & 
    \textbf{B} & \textbf{D} & \textbf{\%} & 
    \textbf{B} & \textbf{D} & \textbf{\%} \\\midrule
    1 & 30 & 7,71\% & 2 &  9 & 97,40\% & 2 & 15 & 98,01\% & 2 & 21 & 97,62\% \\
    2 & 6 & 92,22\% & 2 & 12 & 97,74\% & 2 & 18 & 98,01\% & 3 & 10 & 0,00\% \\\bottomrule
    
    \end{tabular}
\end{table}

\subsection{Model Assisted Calibration of Anomaly Detection} 
\label{ssec:modelbasedinsights}


This section provides insights on the experimental results using the proposed model to define the best parameterization based on system's data.
First, we parameterize the proposed model  from  the experimental data. 
To exemplify the general process, we focus on  the  TRADE\_LOOKUP transaction, for which we  identify  that $p_1$ and $p_2$ equal 0.46 and 0.71, respectively. 
We assess the expected number of samples until a false alarm, obtained from~\eqref{eq:a2p1p2d}, with  $B=2$, $p_1=0.46$,  $p_2=0.71$, and letting $D$ vary between 1 and 30.  For $D=15$, we observed that the number of samples until a false alarm surpasses  $10^7$. 

% \figurename~\ref{fig:modelpar1} is obtained 

\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{bucketfig1.png}
    \caption{Expected number of samples until false alarm,  derived from the proposed analytical model.
    We note that  for $D=15$ the number of samples until a false alarm surpasses   $10^7$.} \label{fig:modelpar1}
\end{figure}

\end{comment}

\begin{figure}[t]
    \centering
    %\includegraphics[width=0.4\textwidth]{prob_fp.pdf}
    \includegraphics[width=\linewidth]{img/prob_fp.pdf}
\caption{Probability of false alarm from model tuned based on  experiments.}
%When $D=12$ the probability of false alarm is already close to 0.}
\label{fig:modelpar2}
\end{figure}

\begin{comment}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{plot4.png}
    \caption{ Cost as a function of bucket depth $(D)$.  Cost is given by $C=w f+ K D$, with $K=2$ and $w=909$, where $f$ is the probability of false alarm. Under the deterministic (resp., exponential) model, cost is minimized for $D=13$ (resp., $D=18$). }
    \label{fig:modelpar3}
\end{figure}

\end{comment}


\figurename~\ref{fig:modelpar2} % and~\ref{fig:modelpar3} 
accounts for an attack model, wherein the mean time between  attacks is $1/\alpha=5 \times 10^5$ samples, i.e., the attack rate is  $\alpha=2 \times  10^{-6}$ attacks per sample.   As the bucket depth increases, the probability of false alarm decreases.   For $D  \ge 12$, the probability of false alarm is  close to 0.

As discussed above, there is a tradeoff between the probability of false alarm and the time to detect attacks once they occur.  To cope with such a tradeoff, we consider both approaches  introduced in Section~\ref{sec:optimization}, namely the hard and soft constraint problems.  
Under the hard constraint problem,  a target probability of false alarm is determined, and the minimum value of $D$ that satisfies such target is sought.  For instance, if we set $F=0.03$ in~\eqref{eq:hard} then the minimum value of $D$ satisfying the constraint is $D=15$ and $D=13$ under the exponential and deterministic attack models, respectively.


\begin{comment}
a simple cost function, which is given by a weighted sum of two terms.  The first term corresponds to the probability of false alarm  and the second  corresponds to the  number of samples necessary to detect an attack once it occurs,  
\begin{equation}
    C(\bm{p}, w, D, K, \alpha)  = f(A_B, \alpha^{-1}) + w K D
\end{equation}
where $w$ is a weight balancing between the two contending aspects.

\end{comment}

We also assess how the cost  $C(\bm{p}, w, D, B, \alpha)$ introduced in Definition~\ref{def:cost}  varies as  a function of $D$,  letting $B=2$, $p_1=0.46$, $p_2=0.71$ and $\alpha=2 \times  10^{-6}$.  Letting $w=909$, which corresponds to the Lagrange multiplier of the constrained problem under the deterministic model (see also~\eqref{eq:lag}),  the optimal bucket depth equals $D=13$, %.  Considering the same parameterization, the optimal bucket depth equals  $D=18$ under the  exponential model,
which is in agreement with the result  presented in the previous paragraph.  Note that for the exponential model the minimum cost is attained at $D=18$, which is slightly larger than $D=15$ obtained in the previous paragraph. This is because the Lagrange multiplier corresponding to the exponential model is $w=57$.  Using such a smaller weight  favors a reduction in the optimal bucket depth to $D=15$, again in agreement with the results discussed in the previous paragraph.  

% depending on whether the deterministic or exponential   models are used  to determine the probability of false alarm as a function of $A_2$.   

\emph{Take away message and engineering implications:}
the analysis presented in this section is instrumental to perform what-if counterfactual analysis and execute utility-driven model parameterization.  If the system administrator implements global countermeasures against attacks, for instance, it is expected that the rate of attacks will decrease. In that case, the bucket depth can be adjusted accordingly, e.g., using the proposed utility-driven approach presented in this section.


% The approach can be initially configured through the mechanism previously illustrated, and then tuned to account  for novel system  setups.


\begin{comment}
Next, we discuss some engineering implications derived from our model-driven analysis of the experimental results.

\textbf{Reverse engineering utility function of existing systems}  
The results presented in this section are instrumental to reverse engineer the utility function subsumed by existing systems.  For instance, consider a system operating with $B=2$ buckets with depth $D=15$. The analysis presented in the previous section shows that this is optimal, for instance, in case $5\times 10^{5}$ samples are collected inbetween attacks and $w=57$, leading to a false positive probability of roughly 0.03.   Knowing that this is the case, one can tune the utility function, e.g., to account for attacks that occur at different rates, and verify when/if the parameters of the bucket algorithm should be adjusted.

\textbf{Counterfactual analysis} As pointed in the previous paragraph, reverse enginneering the utility function is helpful to perform what if analysis and execute utility-driven model parameterization.  If the system administrator implements global countermeasures against attacks, for instance, it is expected that the rate of attacks will decrease. In that case, the bucket depth can be adjusted accordingly, e.g., using the proposed utility-driven approach presented in this section. The approach can be initially configured through the reverse engineering mechanism previously illustrated, and then tuned to account  for novel system  setups.


\end{comment}

\begin{comment}

\clearpage
\pagebreak

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.4\textwidth]{bucketfig1.png}
    
       (a) Expected number of samples until false alarm,  derived from the proposed analytical model.
    We note that   for $D=15$ the number of samples until a false alarm surpasses   $10^7$.
    
    \includegraphics[width=0.4\textwidth]{bucketfig2.png}

(b) Probability of false alarm, under exponential and deterministic models. In both cases, when $D=15$ the probability of false alarm is already close to 0.  

    \includegraphics[width=0.4\textwidth]{bucketfig3.png}
    
    (c) Cost as a function of bucket depth $(D)$.  Cost is given by $C=f+0.018 D$, where $f$ is the probability of false alarm. Under the exponential model, cost is minimized for $D=15$. 

    \caption{    Analytical results derived from parameterized model, letting $K=2$, $p_1=0.46$ and $p_2=0.71$. In parts (b) and (c),  we let the attack rate be given by  $\alpha=2 \times  10^{-6}$ attacks per sample. }
    \label{fig:apfig1}
\end{figure}

\end{comment}



\color{black}


\section{Results and Discussion}
\label{sec:results}

In this section, we first analyze the residual effects that can arise after the attacks and how to identify them. Following, we carry out the analysis of the effectiveness of the anomaly detection approach using two case studies in our environment. 

Our results are discussed using three metrics widely adopted in classification assessment~\cite{zaki2014dataminingbook}, namely  precision, recall and F-measure, which are defined as a function of true positives (TP), false positives (FP) and false negatives (FN) as follows,

\begin{small}
\begin{align}
\textrm{Pr} = \frac{TP}{TP + FP},  \ \ &
\textrm{Re} = \frac{TP}{TP + FN},    &
\textrm{F1} = \frac{2 \times \textrm{Pr} \times \textrm{Re}}{\textrm{Pr} + \textrm{Re}}.  
\label{eq:perf_equa} 
% &= \frac{2 \times TP}{2\times TP + FN + FP}
\end{align}
\end{small}

Precision (Pr) measures the impact of FP in the method's positive prediction.
Recall (Re)  reflects the sensitiveness of the algorithm, capturing the fraction of corrected predictions. 
 F-measure (F1) is the harmonic mean of precision and recall,  balancing them in a single metric. 
 
 % Equation~\eqref{eq:perf_equa} define those metrics.
%
% tirei as virgulas porque pareciam apostrofos na formula anterior


% \label{eq:precision}

\subsection{Residual Effects}
\label{sec:re}

During our experimentation we observed that the number of alerts immediately after the attack phase was significantly higher than in other non-attack period.
We carried an analysis to understand what does it mean the alerts that appear in the post-attack phase.  
We accounted for the number of alarms and the distance, in seconds, from the end of the attack injection phase. 
As \figurename~\ref{fig:re} shows, most of the bucket overflown happens a few seconds after the attack, which suggests that those alerts can be residual effects and not false positives.  

\begin{figure}[htb]
\centering
\vspace{-0.05in}
\includegraphics[width=\linewidth]{./img/alerts_residual.pdf}
\vspace{-0.1in}
\caption{Post-attack alerts distribution for bucket configuration with B=2 and D=[12,15]. Note that x scale is cropped to simplify for more readability.}
\label{fig:re}
\vspace{-0.05in}
\end{figure}

A natural question that arises is what is a reasonable threshold that would discriminate between false positive and residual effects of the attack.  
Regression techniques,  outliers detection techniques, among others, can be used to estimate that threshold. 
In this work, to calculate a reasonable limit without increasing the complexity, we computed the meantime for the first alarm during the attack phase. 
We used it as a threshold estimation to differentiate residual effects from FP.  

In \tableautorefname~\ref{tab:re_thrsd}, we can see the meantime to first attack for two transactions for different bucket's depth. 

\begin{table}[ht]
 %\small
\centering
\vspace{-0.05in}
\caption{ \scriptsize Mean time to first alarm during the attack injection (in seconds)}
\label{tab:re_thrsd}
\begin{tabular}{ccccc}
\toprule
\textit{\textbf{Transaction}} & \textbf{d=6} & \textbf{d=9} & \textbf{d=12} & \textbf{d=15} \\\midrule
TRADE\_LOOKUP & 31,03 & 50,06 & 69,18 & 61,63 \\
MARKET\_WATCH & 36,08 & 54,11 & 60,38 & 59,51 \\\bottomrule
\end{tabular}
\end{table}


We know that, on average, the number of seconds to the \gls{ba} alarm over some constrains (parameters and transaction) is $\delta$.  
We also know that an attack has just ended. 
So, it is reasonable to assume that any alert that occurs in time $t < \delta$  can be associated with residual effects (emptying queues, recovering from errors states, etc.)  of the previous attack, and that is our reasoning behind this approach.


\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{./img/residual_effects.pdf}
    
    \caption{Distribution of the residual effects by failure mode and bucket depth.}
    \label{fig:re_breakdwon}
    \vspace{-0.05in}
\end{figure}


\figurename~\ref{fig:re_breakdwon} shows additional evidences that corroborate with our assumption. 
Only the failure mode with higher (H) intensity induce those alerts. 
When the system is in its peak performance, phase six (blue dashed line), the number of alerts is greater than in the fourth phase. 
Finally, when $D$ increases, the number of alerts decreases, what is expected if those alerts are related to residual effects, since the larger the $D$, the bigger is the tolerance for transient faults.

\vspace{-0.06in}
\subsection{Case Study 1}

In our first case study, we will assess the detection effectiveness of the \gls{ba} over our fault models and how the parameterization affects the method's performance. 
Here we will use the same parameterization for all operations.
The optimal $D$ value, accordingly with our calibrated model, resides between 12 and 15. 
\tableautorefname~\ref{tab:cs1_tbl} shows the metrics our tests, segmented by different failure modes, and for {\it ALL} failure modes mixed. 

\begin{table}[ht]
    \tiny
    \vspace{-0.1in}
    \centering
    \caption{Metrics values for $D=(12|15)$ of CS1. Maximal value for \textbf{TP} would be 21 for each failure mode and 126 for \textbf{ALL}. }
    \vspace{-0.1in}
    %Table also shows the Residual Effects counts (\textbf{RE}) and \textbf{Pr}ecision, \textbf{Re}call and F-measure (\textbf{F1}) metrics}
    \label{tab:cs1_tbl}
    \includegraphics[width=0.9\linewidth]{./img/cs1_tbl.pdf}
    
\end{table}


The first observation from \tableautorefname~\ref{tab:cs1_tbl} is the method's low number of alerts outside of an attack.  Since we count every alert as an FP, the possibles number of this category could be much higher since we are accounting $4\times 9$ buckets at the same time.  Following, we can note that the \gls{ba} is not useful, in general,  for short attacks with low-intensity, the except is the 6Ls at $D=12$, but it has a worse result compared with the others failure modes. Conversely, to others failure-modes, the method is very effective, even with an f-measure of 1 for the 6H at $D=12$. 


% \begin{figure}[htb]
% \centering
% \includegraphics[width=\linewidth]{./img/precision.pdf}
% \caption{ \scriptsize 
% Campaign Precision for all falt models using two buckets. The data are shown with the  pre and pos phases splitted into two sets.}
% \label{fig:precision}
% \end{figure}


\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{./img/all_metrics.pdf}
\caption{Campaign Precision for all falt models using two buckets. The data are shown with the  pre and pos phases splitted into two sets.}
\vspace{-0.2in}
\label{fig:all_metrics}
\end{figure}

Another question that we tried to answer is what is the impact of the bucket depth on the target metrics (Equation~\ref{eq:perf_equa})? \figurename~\ref{fig:all_metrics} shows the results. Reinforcing our previous observation, the \textit{Ls} failure mode do not perform and are responsible for the small values on those charts. 

A general observation that we can get from the Precision and Recall charts in this analysis is that those metrics have different relations with the bucket depth.  Precision increases with $D$ as the Recall decreases. In this case, the F-measure is an excellent way to balance the method's efficiency. Comparing the different bucket depth, the precision and recall will vary for the distinct failure modes.

% 
% \begin{figure}[htb]
% \centering
% \includegraphics[width=\linewidth]{./img/recall.pdf}
% \caption{ \scriptsize Campaing Recall for two bucket configuration}
% \label{fig:recall}
% \end{figure}



Considering that, ideally, a method should work for every kind of attack, in this case study, $D=12$ provides better results (All curve). But obviously, this is not the case for every system, and one should balance the parameters to get ideal performance, which reinforces the importance of our analytical model and tuning the method by each transaction. 


% \begin{figure}[htb]
% \centering
% \includegraphics[width=\linewidth]{./img/f_measure.pdf}
% \caption{ \scriptsize F-Measure across the different fault models for both phases under evaluation.}
% \label{fig:f1}
% \end{figure}

\subsection{Case Study 2}

We have seen in \tableautorefname~\ref{tab:basel_alert_txns} that not every transaction has similar configuration. A natural assumption is that different parameterization for each operation should lead to better performance.  To validate that intuition, based on the cited table, we created a mix (Mix 6/9/12/15) of parameterization in which we use the first null $D$ value for each transaction. \tableautorefname~\ref{tab:cs2_tbl} show the results. 

Despite being a better positive predictive setup, it almost tripled the number of FP which greatly penalize the overall performance of the configuration. Those transactions with lower bucket depth cause this higher number of FP. 


\begin{table}[ht]
    \tiny
    \centering
\caption{ \scriptsize Result of Case Study 2, showing the Residual Effects counts (\textbf{RE}), \textbf{Pr}ecision, \textbf{Re}call and F-measure (\textbf{F1}) metrics}
    \label{tab:cs2_tbl}
    \includegraphics[width=0.9\linewidth]{./img/cs2_tbl.pdf}
\end{table}

As a next tunning, following our analytical model, we avoided the values of $D$ below 12, just raised the values of 6 and 9 to 12. The results are, also shown on \tableautorefname~\ref{tab:cs2_tbl}.  

In general, the performance is increased, especially for the {\it L} cases. The exception is the {\it Ls} failure mode, that we already now that are not well covered by the method. 






\section{Threats to Validity}
\label{sec:threats}

% \toNA{\cg{Nem tudo ai pode fazer sentido, estou so fazendo um brainstorm para depois iterar sobre}}

Next, we discuss some of the  assumptions considered in this paper and their implications. 

 \emph{Fault model representativeness}: %  as in any experimental exercise, we had to trade between simplicity and representativeness. To that aim, we considered a database  workload, namely the TPCx-V benchmark.  Then, 
 the faults injected in the system are  generated by stressing the underlying OS. In real systems, different attacks may produce various effects on multiple layers of the system stack.  Nonetheless, as far as the subsumed OS states resulting from those attacks correspond to states generated by our fault injection, the  considered failures are representative of those that occur in  systems under operation~\cite{arlat1990fault, arlat_dependability_2002}. 
 
%  For that reason, one can argue about the representativeness of those faults.   But this limitation is minimized since the observed state of the system characterizes a 
 
 
\begin{comment}
 
 
  \emph{Target environment and workload}: As in any experimental exercise, we had to trade between simplicity and representativeness. To that aim, we considered a database  workload, namely the TPCx-V benchmark.  We envision that our experiments can be easily extended to other workloads, and leave that as subject for future work. %  and some of its related metrics the throughput capacity and is not generic.
 
 \emph{Assessment at scale}: we consider system-wide global detection of anomalies. Alternatively, one can consider  segmented anomaly detection for subsystems inside the considered ecosystem.  The nuts and bolts of how to combine the results of multiple anomaly detection instances per subsystem are out of the scope of this work, although such assessment is contemplated  by  the proposed methodology.  
 
\end{comment} 
 
%  thus restrict the applicability. Nevertheless, such an assessment is possible within this methodology.
  
  \emph{Profile obsolescence:} if user profiles are not stable,  %if the operational profile changes, 
  the number of false alerts can increase significantly, making the detection system useless until the next iteration. In that case, time must be divided into windows and the solution presented in this paper needs to  be applied and tuned at every  window.  To determine the optimal window size  one may rely on techniques for learning in non-stationary environments~\cite{sayed2012learning}.
  
  
  
%  can be challenges for some systems that do not have a stable operational profile. 
  
  %  \emph{Obsolescence}: if the operational profile changes, the number of false alerts can increase significantly, making the detection system useless until the next iteration.

 \emph{Covert degradation}: single metrics  may not suffice to detect anomalies.  A detector  using response time as its metric, for instance,  may miss-detect attacks that impair  system availability if the few transactions that succeed to  complete have their response time within  the expected  range.  A similar effect occurs  with respect to  throughput in elastic systems. This limitation can be mitigated using multiple complementary metrics for anomaly detection.





\section{Conclusion} 
\label{conc}

In this work, we presented a methodology for anomaly detection based on performance degradation caused by security attacks for complex virtualized systems.  The approach leverages an analytical model to optimize the detection technique in a principled way. % and was designed to allow  integration into the daily operation and adapt to system's changes.  
Our experimental assessment indicates the method's effectiveness by  injecting resource exhaustion attacks in a complex virtualized system. Results show that it is possible to detect anomalous behavior using  the throughput of the business transactions with an average precision of 90\% and recall of 86\%.  Our experimental results also bring awareness about residual effects of  high-intensity fault loads, which may persist for a significant amount of time after the active attack has been interrupted. Such residual effects  give rise to false positives,  further motivating the use of analytical models to  tune the false positive rate in a principled  fashion.

% During our experimental campaign, we were able to differentiate the residual effects of high-intensity fault loads.




==> 2019_dsn_submitted/customCommands.tex <==
\newcommand*{\TPC}{\texttt{TPCx-V}}
%\newcommand*{\TPC}{\texttt{TPCx-V}\xspace}

\newcommand*{\fmU}{\textit{UNKNOWN\_ERROR}\xspace}
\newcommand*{\fmS}{\textit{SUCCESS}\xspace}
\newcommand*{\fmC}{\textit{GUEST\_CRASH}\xspace}
\newcommand*{\fmK}{\textit{GUEST\_KILL}\xspace}
\newcommand*{\fmGH}{\textit{GUEST\_HANG}\xspace}
\newcommand*{\fmE}{\textit{ERROR}\xspace}
\newcommand*{\fmIH}{\textit{INJECTION\_HANG}\xspace}


\newcommand\Mark[1]{\textsuperscript{#1}}    


==> 2019_dsn_submitted/experiments.tex <==
\subsection{Experiment $\alpha$}

This experiment is based on the following Golden Runs
\begin{quote}
\textit{ 279 280 281 282 284 285 286 287\\
288 289 290 291 292 293 295}
\end{quote}


\subsection{Applying the Bucket in our environment}
\toCG{How we compute the average and standard deviation}
\toCG{How we apply the BA in our environment}


\subsection{False Positives Analysis}

Based on the profile estimated for the $alpha$ experiment, for each transaction we 
counted the number of alerts.



\subsection{Research Questions}

\begin{itemize}
\item Could a customer-affecting performance metric be used to assess the impact of fault 
injection in virtualized environments?

\item What is the best parametrization (\textit{b}$\times$\textit{d}) to use in our 
context ?



\subsection{Run06}

\toCG{What was the initial idea of tests? Test Everything that did not (usually) cause 
restart or crash. For this we will use randomly selected groups of 6000 tests for the 
\fmS and \fmU} 
% Check http://localhost:8888/notebooks/notes/Attack%20Runs.ipynb
\toCG{We are looking for any sign of anomaly during the execution. The trivial signs
of inadequacy was already detected. Since we perform non expected behavior, and given 
that there is no formal proof that the Xen is bug free, any fault must be activated. Even 
if the failure are not clearly detected}


The test that generated a clear unexpected behavior was the test 06. Based on our 
previous work we only selected tests that was initially categorized having a failure mode 
as \fmS or \fmU. We already know that some tests a failure mode that are not 
deterministic. In fact in our previous work we were analyzing the individual effect 
of each test, and we concluded that they are not as deterministic as expected. That way, 
running the test 06 multiple times led to the observation of many of our defined failure 
modes. 

\toCG{Create a table with all of them. Up to now: \\
       25 \fmC \\
        5 \fmGH \\ 
        1 \fmIH \\ 
     7670 \fmS \\ 
       12 \fmU
}


During the testing campaign in the Run06, we sequentially injected the malicious 
hypercalls in the \gls{ct} monitoring the environment to detect which failure is 
observed. When a \fmC or \fmK occurs the \gls{tm} restart the \gls{ct} and ensure the base
workload on it. With a relative frequency ($>$ 70\%) a stall with approximately 2 hours
on this process occur. This behavior is not observed in any other test, neither on those 
composed purely of \fmC or \fmK which mitigates the risk of this being caused by a bug 
on the \gls{tm}. 

After a careful manual analysis we detected that the freeze was happening during the 
remote invocation (using ssh) of the background workload. Using the hypervisor console we 
detected a recurrent warning of a soft lockup in both CPU  (\textit{rcu\_sched} stall). 
Using the process monitor tool by Xen we can see that the CPU usage are at full rate 
(200\%), the host respond to ping normally.



\end{itemize}

 


==> 2019_dsn_submitted/glossary.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Acronyms (example below)
% Usage: \gls{link]   |  \glspl{link} (plural)
% \newacronym{link}{INITIALS}{Description of Initials}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{glossaries}

\newacronym[plural=CPUs,firstplural=Central Processing Units (CPUs)]{cpu}{CPU}{Central Processing Unit}
\newacronym[plural=HVMs,firstplural=Hardware Virtual Machines (HVMs)]{hvm}{HVM}{Hardware Virtual Machine}
\newacronym[plural=IDSes,firstplural=Intrusion Detection Systems (IDSes)]{ids}{IDS}{Intrusion Detection System}
\newacronym[plural=LKMs,firstplural=Loadable Kernel Modules (LKMs)]{lkm}{LKM}{Loadable Kernel Module}
\newacronym[plural=OSes,firstplural=Operating Systems (OSes)]{os}{OS}{Operating System}
\newacronym[plural=vCPUs,firstplural=Virtual CPUs (vCPUs)]{vcpu}{vCPU}{Virtual CPU}
\newacronym[plural=VMs,firstplural=Virtual Machines (VMs)]{vm}{VM}{Virtual Machine}

\newacronym{api}{API}{Application Programming Interface}
\newacronym{ba}{$BA$}{Bucket Algorithm}

\newacronym{cisuc}{CISUC}{Center for Informatics and Systems of the University of Coimbra}
\newacronym{ct}{CT}{Compromised Tenant}
\newacronym{db}{DB}{Dependability Benchmark}
\newacronym{dos}{DoS}{Denial-of-service}
\newacronym{dei}{DEI}{Department Informatics Engineering}
\newacronym{gdt}{GDT}{Global Descriptor Table}
\newacronym{iaas}{IaaS}{Infrastructure as a Service}
\newacronym{kvm}{KVM}{Kernel-based Virtual Machine}
\newacronym{mafalda}{MAFALDA}{Microkernel Assessment by Fault injection AnaLysis and Design Aid}
\newacronym{mcdm}{MCDM}{Multi-Criteria Decision Making}
\newacronym{oltp}{OLTP}{Online Transaction Processing}
\newacronym{pb}{PB}{Performance Benchmark}
\newacronym{pv}{PV}{Paravirtualization}
\newacronym{qa}{QAs}{Quality Attributes}
\newacronym{qm}{QM}{Quality Model}
\newacronym{rq}{RQ}{Research Question}
\newacronym{sb}{SB}{Security Benchmark}
\newacronym{spec}{SPEC}{System Performance Evaluation Cooperative}
\newacronym{sut}{SUT}{System Under Test}
\newacronym{tm}{TM}{Test Manager}

\newacronym{tpcxv}{\TPC}{TPC Express Benchmark V~\cite{TPCx-V_spec}}
\newacronym{tpc}{TPC}{Transaction Processing Performance Council}
\newacronym{vi}{VI}{Virtualization Infrastructures}
\newacronym{vmi}{VMI}{Virtual Machine Introspection}
\newacronym{vmm}{VMM}{Virtual Machine Monitor}
\newacronym{wg}{WG}{Working Group}
\newacronym{wsdl}{WSDL}{Web Services Description Language}


% 
% \newacronym[plural=VMs,firstplural=Virtual Machines (VMs)]{vm}{VM}{Virtual Machine}
% \newacronym[plural=HVMs,firstplural=Hardware Virtual Machines (HVMs)]{hvm}{HVM}{Hardware Virtual Machine}
% \newacronym{pv}{PV}{Paravirtualization}
% \newacronym[plural=OSes,firstplural=Operating Systems (OSes)]{os}{OS}{Operating System}
% %\newacronym{vmm}{VMM}{Virtual Machine Monitor}
% \newacronym{kvm}{KVM}{Kernel-based Virtual Machine}% 
% \newacronym{gdt}{GDT}{Global Descriptor Table}
% \newacronym{api}{API}{Application Programming Interface}
% \newacronym{wsdl}{WSDL}{Web Services Description Language}
% \newacronym[plural=IDSes,firstplural=Intrusion Detection Systems (IDSes)]{ids}{IDS}{Intrusion Detection System}
% \newacronym[plural=LKMs,firstplural=Loadable Kernel Modules (LKMs)]{lkm}{LKM}{Loadable Kernel Module}
% \newacronym{vmi}{VMI}{Virtual Machine Introspection}
% \newacronym[plural=CPUs,firstplural=Central Processing Units (CPUs)]{cpu}{CPU}{Central Processing Unit}
% \newacronym[plural=vCPUs,firstplural=Virtual CPUs (vCPUs)]{vcpu}{vCPU}{Virtual CPU}
% \newacronym{mafalda}{MAFALDA}{Microkernel Assessment by Fault injection AnaLysis and Design Aid}
% \newacronym[plural=,firstplural= ()]{}{}{}




%\newacronym{tpc}{}{}
%Use GLS
\glsresetall


==> 2019_dsn_submitted/outline.tex <==
\section{Introduction}
\toAA{Focus on Introduction}
\toCG{virtualization / Multi-tenancy / }
\toCG{Complex environments for subtle problems;}
\toCG{Performance modeling in security and anomaly, overcommit;}
\toCG{Can Performance Modeling help in this context?}
\toCG{Goals and Finding}

% ------------------------------------------------------------------------------------------------
\section{Related Work}
\toAA{performance monitoring}
\toDM{Random Walk References}
\toCG{resource exhaustion}
\toCG{metrics to detect anomalies}
\toCG{Cite related \gls{tpcxv} work to introduce the high level details}

% ------------------------------------------------------------------------------------------------
\section{Methodology}
\toCG{Create a diagram to summarize the methodology}
\toCG{Golden Runs}
\toCG{Baseline parameters estimation}
\toCG{B x D estimation}
\toCG{Explain how we pretend to compare the results}


\subsection{Fault Model}
\toCG{types of "attacks" H | L | Ls}
\toCG{Test phase Specifications (4 and 6 )}

\subsection{Adapting the Bucket Algorithm}
\toCG{Explain how we adapted the BA, the alert definitions based on multiple diferent transactions/buckets}
\toCG{Detecting Positives Alerts}



% ------------------------------------------------------------------------------------------------
\section{Performance Degradation Detection Algorithm} 
\toCG{Bucket Algorithm details}



% ------------------------------------------------------------------------------------------------
\section{Experimental Virtualized Environment} 

\subsection{\gls{tpcxv}}
\toCG{Explain relevant technical details of \gls{tpcxv}}
\subsection{Experimental Setup}
\toCG{Explain our setup, deployment}


% ------------------------------------------------------------------------------------------------
\section{Experimental Campaign}
\toCG{Number of runs, run duration, automation process}
\toCG{Explain that not every Txn contributes for the}
\toCG{Response Time vs Throughput databases}
\toCG{Table showing the  }
\toCG{B x D estimation data}
% ------------------------------------------------------------------------------------------------
\section{Results and Discussion}
\toCG{Baseline Validation}
\toCG{TP / FP and Precision / Recall}
\subsection{Analysis}
\toDM{Discuss the Random Walk Model and analysis here}

% ------------------------------------------------------------------------------------------------
\section{Conclusion}
\toCG{summarize the paper contribution}
\section*{Contributions Discussion}
\cg{Just a \textit{Reminder} Subsection to summarize main contributions while writing}
\begin{enumerate}
 \item A methodology to apply the bucket Algorithm in a complex system and its instantiation
 \item 
\end{enumerate}



==> 2020_001_framework.tex <==

    \section{Attack Detection Methodology} 
    \label{sec:meth}
    
This section describes the proposed attack detection approach, which has the goal of helping the users to successfully apply our anomaly detection algorithm into the life cycle of their systems. An essential aspect of an anomaly detection approach is to be able to cope with changes in the operational profile, as the monitored systems commonly have different loads and demands over time. 
Our methodology follows a cyclic approach and foresees additional iterations to accommodate each new operational profile.  
    \figurename~\ref{fig:meth_lc} depicts the high-level application of the methodology.
    
    \setcounter{figure}{0} % aldrabice por causa das figuras
    
    \begin{figure}[ht]
        \centering
        \includegraphics[width=\linewidth]{./img/meth_lc.pdf}
        \caption{Overview of the methodology application life cycle.}
        \label{fig:meth_lc}
        %\vspace{-5pt}
    \end{figure}
    
    \setcounter{figure}{2} % aldrabice por causa das figuras
    
    
    As we can observe, the methodology consists of three main phases: 
    \textbf{(A) exploratory analysis}, which allows determining the most effective way to monitor the system based on its characteristics; 
    \textbf{(B) profiling}, which evaluates the system on its expected regular operational profile(s)~\cite{Musa1993} to extract information about the habitual behavior and its performance;
    and \textbf{(C) Operation}, in which the system executes for its intended purposes, and we use all data and knowledge from the previous phases and report deviations, identifying them as anomalies or attacks. 
    
    A new iteration is needed if changes are detected: 
    $i)$ in the system, demanding a new complete iteration to see if there are relevant aspects to add to the monitoring surface,
    $ii)$ in the operational profile, requiring to repeat the profiling. This does not mean that the previous parameters are obsolete, it could represent a profile change that can be expected within some periodicity (e.g. holiday/promotion seasons). 
    
    The phases of methodology are detailed in  \figurename~\ref{fig:meth}, and explained in the ensuing sections.
    
    
    %An application of this method leads to a monitoring cycle that,  during the daily system operation ($C_{1}$), allows the user to detect attacks ($C_{2}$) by getting alerts ($C_{3}$) and take action ($C_{4}$) to establish the regular operation. 
    %Also, the methodology can be integrated into the system's life cycle and adapted to routinely incorporate the changes that occur in the system's operational profile. 
    
    
    
    
    \subsection{Exploratory analysis phase}
    
    This phase has the objective of determining the monitoring surface used to monitor the system's performance.  
    To achieve that goal, the user needs to follow three main steps:  
    
    $A.1)$ \emph{Analysis:} evaluate the system's internal aspects like its architecture, components, operations and resources that are available for monitoring to define how to characterize the system performance
     
    $A.2)$ \emph{Exploration:} the tacit knowledge of the system is essential, and a set of executions of the system (\textbf{E} on \figurename~\ref{fig:meth}) is prescribed for exploratory analysis. 
    During those executions,  all monitored data should be collected and analyzed  to understand the metrics that effectively translate into useful measurements;
    
    $A.3)$  \emph{Definition:} use previous steps to determine the \textbf{monitoring surface}. The monitoring surface analysis is the effort of joining the tacit knowledge and internal aspects to define which components and metrics to use in the following phases. 
    
    
    \subsection{Profiling phase}
    
    %\nuno{WiP: evaluate the environment under execution on its regular operational profile (a quantitative characterization of how a system will be used~\cite{Musa1993}) to extract information about the expected behavior and the optimal way of assessing the performance of the system}
    
    %  regular operational profile(s)
    
    This phase has the objective of evaluating the environment during the execution of its expected regular operational profiles~\cite{Musa1993}, in order to establish the statistical parameters that represent those profiles. 
    The following procedures are needed: 
    
    $B.1)$ \emph{Golden runs definition:} the system is exercised under usual operational conditions, i.e., without any fault/attack to collect the available data using the monitor surface. 
    These system's executions are called \textbf{golden runs} and are the primary reference for the system's normal behavior.  
    We split them into two independent sets: one \textbf{P}rofile set used to compute the baseline metrics, and the second set used to \textbf{V}alidate the performance parameterization.
    
     
    $B.2)$ \emph{Baseline metrics extraction:} the computation of the baseline metrics is conducted extracting statistical data from the metrics defined over the monitoring surface. 
    Those extractions should be made for each subsystem, metric, operation and resource, and operational profile. 
    
    % The computation of the baseline metrics is defined accordingly with the performance monitoring algorithm used.  Those metrics should be set for each subsystem, metric, transaction, and operational profile.
    
    % Once the baseline metrics are established, we are ready to calibrate the performance model using the empirical data generated. We run several experiments using the Golden Runs data and the detection algorithm with different configurations. The performance model determines which parameters are best suitable for the tests.  We, then, account for the number of alerts that a given setting will cause.  Since we are assessing experimental runs under no attack conditions, we can define the algorithm tolerance for the number of false positives accordingly with the user's threshold goal.  The performance model will assist in minimizing the false positive rate. The calibrated performance model is the algorithm parameterization that is best suitable for the system-specific detection goals.
    
    % The final step is the baseline validation to check the validity of the determined parameters. We run the detection algorithm with the Golden Runs from the \textbf{V} group and check if the number of alerts (false positives) is in the defined experiment criteria.  If this is not the case, we can go back to the recalibrate the performance model until the requirements are fulfilled.
    
    
    $B.3)$ \emph{Performance model calibration:} apply the empirical data to determine the optimal values that minimize the false positives (FP) alerts. 
    The performance model determines which parameters are best suitable for the tests.  
    Then, we account for the number of alerts that a given setting will cause.  
    As we are assessing experimental runs under no attack conditions, we can define the algorithm tolerance for the number of FPs according to the user's preference.
    The performance model will assist in minimizing the FP rate. 
     
    $B.4)$ \emph{Baseline validation:} check the validity of the determined parameters. Apply the detection algorithm using the Golden Runs from the \textbf{V} group and check if the number of alerts (FP) is in the defined experiment criteria.  
    
    $B.5)$ \emph{Parameterization adjustment:}  during the baseline validation, if the alert rate does not meet the defined objective, we can go back and recalibrate the performance model until the requirements are met.
    
    
    
    \subsection{Operation phase}
    \label{sec:met_op}
    
    % \nuno{wip: Finally, on the Operation step, we use all data and knowledge from the previous components to search for anomalies or attacks during the system operation. }
    
    At this point, the anomaly detection algorithm is fully configured to monitor the system in production and detect security attacks that cause performance degradation. 
    Thus, in this phase, we take advantage of all the data and knowledge from the previous components to search for anomalies or attacks during the system operation.
    We need to:
    
    $C.1)$ \emph{Define a criterion:} that determines an alert condition in a concise manner. For instance, every alarm in any transaction or only alerts in critical subsystems?
    
    $C.2)$ \emph{Monitor the operation:} integrate the detection algorithm into the daily activity by continually watching  the monitoring surface using the detection algorithm with the optimal parameters
    
    
    
    


==> 2020_002_threats.tex <==


\section{Threats to Validity}
\label{sec:threats}

% \toNA{\cg{Nem tudo ai pode fazer sentido, estou so fazendo um brainstorm para depois iterar sobre}}

Next, we discuss some of the  assumptions considered in this paper and their implications. 

 \emph{Fault model representativeness}: %  as in any experimental exercise, we had to trade between simplicity and representativeness. To that aim, we considered a database  workload, namely the TPCx-V benchmark.  Then, 
 the faults injected in the system are  generated by stressing the underlying OS. In real systems, different attacks may produce various effects on multiple layers of the system stack.  Nonetheless, as far as the subsumed OS states resulting from those attacks correspond to states generated by our fault injection, the  considered failures are representative of those that occur in  systems under operation~\cite{arlat1990fault, arlat_dependability_2002}. 
 
%  For that reason, one can argue about the representativeness of those faults.   But this limitation is minimized since the observed state of the system characterizes a 
 
 
\begin{comment}
 
 
  \emph{Target environment and workload}: As in any experimental exercise, we had to trade between simplicity and representativeness. To that aim, we considered a database  workload, namely the TPCx-V benchmark.  We envision that our experiments can be easily extended to other workloads, and leave that as subject for future work. %  and some of its related metrics the throughput capacity and is not generic.
 
 \emph{Assessment at scale}: we consider system-wide global detection of anomalies. Alternatively, one can consider  segmented anomaly detection for subsystems inside the considered ecosystem.  The nuts and bolts of how to combine the results of multiple anomaly detection instances per subsystem are out of the scope of this work, although such assessment is contemplated  by  the proposed methodology.  
 
\end{comment} 
 
%  thus restrict the applicability. Nevertheless, such an assessment is possible within this methodology.
  
  \emph{Profile obsolescence:} if user profiles are not stable,  %if the operational profile changes, 
  the number of false alerts can increase significantly, making the detection system useless until the next iteration. In that case, time must be divided into windows and the solution presented in this paper needs to  be applied and tuned at every  window.  To determine the optimal window size  one may rely on techniques for learning in non-stationary environments~\cite{sayed2012learning}.
  
  
  
%  can be challenges for some systems that do not have a stable operational profile. 
  
  %  \emph{Obsolescence}: if the operational profile changes, the number of false alerts can increase significantly, making the detection system useless until the next iteration.

 \emph{Covert degradation}: single metrics  may not suffice to detect anomalies.  A detector  using response time as its metric, for instance,  may miss-detect attacks that impair  system availability if the few transactions that succeed to  complete have their response time within  the expected  range.  A similar effect occurs  with respect to  throughput in elastic systems. This limitation can be mitigated using multiple complementary metrics for anomaly detection.




==> 2020_003_exploratory_etal.tex <==


\subsection{Exploratory Phase}
\label{ssec:sut-exploratory}

%The first part was to understand the  \gls{tpcxv} architecture, and its specification to get some tacit knowledge about its deployment in our environment.  
In previous works~\cite{AvritzerBGTW06,avritzer2010monitoring},  the \gls{ba} was applied using response time as the anomaly detection metric. 
In this work, we are evaluating a complex system with different components and subsystems that aims to maximize its throughput. 
Hence, we decided to  use the system's throughput as the input metric for the \gls{ba}.   

Based on the response time data available from the \gls{tpcxv} results, we derived a throughput extraction process that aggregates the transactions by group, phase, transaction type, and  the operation completion time. 
To accommodate a metric that is best when its value is short (contrary to the response time), we updated the algorithm accordingly. 
It will penalize the metric if its value is lower than the average plus a multiple of the standard deviation, i.e., $\hat{x} < (\mu + (b-1) \sigma)$.

The next step was to perform transaction characterization using  exploratory runs.  A preliminary assessment was made by applying  the \gls{ba} to the collected data.
The analysis revealed that not all of the \gls{tpcxv}'s transactions are useful in reflecting the system's load. 
Additionally, the response time results  evaluation showed  a higher number of false alarms.

To conclude the exploratory phase, we defined our monitoring surface as the throughput information of \texttt{9} (of the \texttt{12}) transactions from \gls{tpcxv}. 
That data was evaluated distinctly for every subsystem (the \texttt{4} \gls{tpcxv}'s groups), resulting in \texttt{36} (\texttt{9x4}) bucket algorithms running, each with \texttt{10} distinct configurations, \texttt{1} for each distinct operation profile (the \texttt{10} \gls{tpcxv}'s phases). 


% After evaluating the algorithm using both metrics, we rapidly noticed that by using the throughput data, we have better results as \tableautorefname~\ref{tab:rtVsTput} shows.  Additionally, some results are different. For instance, in the run 595 (6H), we did not alert in the injection period using the RT, but it did report using the throughput database.

% \begin{table}[ht]
% \normalsize
% \centering
% \caption{Performance comparison for b=2 and d=15}
% \label{tab:rtVsTput}
% \begin{tabular}{cccc}
% \toprule
% & \textbf{TP} & \textbf{FP} & \textbf{Precision\footnotemark[1]} \\ \midrule
% Response Time & 182 & 522 & 25,85\% \\
% Throughput & 1874 & 38 & 98,01\% \\ 
% \bottomrule
% \end{tabular}
% \end{table}
% 
% \footnotetext[1]{For this precision account we simply counted the number of alerts inside and outside the attack period.}


\subsection{Profiling Phase}
\label{ssec:sut-profiling}

To profile the system, we executed 59 golden runs to generate data for the characterization of the system's baseline behavior (37 runs, {\it P set}) and also validation (22 runs, {\it V set}).  
For every transaction from the monitoring surface, we compute and store the average throughput for each subsystem in every operational profile.   
These values are the system's baseline metrics. 

To calibrate our performance model (Section~\ref{ssec:modelbasedinsights}), we need to account for the following metrics:  
\begin{enumerate}
    \item The probability of a false positive alarm as a function of bucket depth;
    \item The probability for each transition in the DTMC (\figurename~\ref{fig:dtmc});
    \item The mean time to first alarm during an attack.
\end{enumerate}

To compute those probabilities, we applied the \gls{ba} with different configurations over the {\it V set} runs data. 
These results are presented in Section~\ref{sec:results}.

For the validation process, we applied the \gls{ba} for every golden run, accounting for the number of alerts (false positives). 
The goal of this step is to check if using the parameters suggested by the model will not generate an unacceptable amount of false-positive alerts.
First, we execute the assessment with the same runs used to generate the baseline metrics ({\it B set}). 
Here we are not validating, only producing values to compare later with the validation results.  
Also, this step can be used for consistency check and to test for possible computational errors, if the results show any abnormal number of alerts. 
Then, we repeat the process using the validation runs ({\it V set}). 
The results of both sets are not significantly different, and thus we present only the validation values in~\tableautorefname~\ref{tab:basel_param}.

The results described in \tableautorefname~\ref{tab:basel_param} show that using two buckets is more effective, as it shows a fair number of false-positive alerts. 
One bucket has too many alerts, and three is likely to be ineffective.

\begin{table}[ht]
%\small
\vspace{-0.1in}
\centering
\caption{\scriptsize  False positive alerts: total count and average ($\mu$) by run in validation}
\label{tab:basel_param}
\vspace{-0.05in}
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{cccc||cccc||cccc}
\toprule
\textbf{B} & \textbf{D} & \textbf{\# Alerts} & \boldmath$\mu$  
& \textbf{B} & \textbf{D} & \textbf{\# Alerts} &  \boldmath$\mu$ 
& \textbf{B} & \textbf{D} & \textbf{\# Alerts} & \boldmath$\mu$  \\\midrule

1 & 30 & 27373 & 1244,23 & 2 & 12 & 4 & 0,18 & 2 & 21 & 0 & 0,00 \\
2 & 6 & 185 & 8,41 & 2 & 15 & 0 & 0,00 & 3 & 10 & 0 & 0 \\
2 & 9 & 12 & 0,55 & 2 & 18 & 0 & 0,00 & & & & \\\bottomrule
\end{tabular}
\end{table}


Looking at the \tableautorefname~\ref{tab:basel_alert_txns}, we can see that for distinct transaction types, we have distinct sensitiveness for the same parameterization, when applying the \gls{ba}.  These distinct sensitivities can suggest that different values for $D$ should be applied for different operations.

\begin{table}[ht]
%\small
\vspace{-0.1in}
\centering
\caption{\scriptsize  False positive alerts segmented by \gls{tpcxv}'s transactions }
\label{tab:basel_alert_txns}
\vspace{-0.05in}
\begin{tabular}{cc|ccccccccc}
\toprule
\multicolumn{2}{c|}{ \textbf{Transaction ID} } & 0 & 1 & 2 & 4 & 5 & 6 & 7 & 8 & 9 \\
\midrule
\multirow{3}{*}{ \textbf{D} } & 6 & 23 & 43 & 28 & 34 & 12 & 23 & 14 & 2 & 6 \\
& 9 & 0 & 1 & 4 & 6 & 1 & 0 & 0 & 0 & 0 \\
& 12 & 0 & 0 & 2 & 2 & 0 & 0 & 0 & 0 & 0 \\\bottomrule
\end{tabular}
\end{table}


When running the \gls{ba} in both golden runs sets, we obtain similar results. This similarity indicates that the profile derived from the baseline metrics can be generalized for different runs.

After the previous analyses, we were able to apply the performance model to the experimental data. Section~\ref{ssec:modelbasedinsights}  contains the process details. The calibrated performance model suggests that bucket depth $D$ shall be configured in the range, $D \in (12,15]$, because the number of false positive alerts within this range is acceptable. 




\subsection{Operational Phase}
\label{ssec:sut-operational}

%In this experimental campaign, we will adapt the methodology operation step to perform an empirical study of the \gls{ba} applicability.

As prescribed in Section~\ref{sec:met_op}, we have to define our alert reporting criteria.  
We adopted distinct approaches to detect \textit{true positives} (TPs) and \textit{false positives} (FPs).  
A TP is when we detect {\bf at least one alert on the attack phase}. 
We only need one alert in any group for any transaction type. 
Complementarily, a \textit{False Negative} (FN) is when \textbf{no alert is raised} on the same phase.  
We consider a FP \textbf{every bucket overflow that happen in the no-attack phase}. 
In this case, two bucket overflows in distinct transactions, or even in the same, but in different groups, will account for two distinct FPs. 
This approach is justified, because alarm systems are required to minimize the number of false positives. 

An alert on the post-attack phase can be a FP or a residual effect caused by the faultload. 
This question will be discussed in Section~\ref{sec:re}.

At last, the \textit{true negative} (TN) does not need  be defined, because the goal of this paper is to apply the \gls{ba} algorithm to continuously detect performance metric deviations during system 
attacks.
%To estimate the number of possible alerts during a specific period, based on a fixed detection window, does not make sense when comparing different workloads and configurations (see Section~\ref{sec:param_ad}).

During the testing campaign process, each of our test runs is composed of three phases, as depicted in \figurename~\ref{fig:testDesc}.  
In those defined periods, we will count the number of FP, TP, and FN as described early. 
Each alert on the post-attack phase will count as a {\it residual effect}.  
When executing the \gls{tpcxv} workload, we will run just one attack, as defined in Section~\ref{ssec:faults}. 
As showed in \tableautorefname~\ref{tab:runs}, we performed 21 runs for each fault injection type, while applying the \gls{ba} throughout the monitoring surface.

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{./img/test_desc_v2.pdf}
    \caption{Distinct phases and its alerts meaning during a test run.}
    \label{fig:testDesc}
\end{figure}

\begin{table}[ht]
    \vspace{-0.1in}
    %\small
    \centering
    \caption{Runs in Experimental Campaign}
    \label{tab:runs}
    \vspace{-0.05in}
    \begin{tabular}{c||cccccc||c}
    \toprule
    Test & 4H & 4L & 4Ls & 6H & 6L & 6Ls & Golden \\
    $N^{o}$ Runs & 21 & 21 & 21 & 21 & 21 & 21 & 59 \\\bottomrule
    \end{tabular}
\end{table}


After the test executions, we used the data collected to apply the \gls{ba} with different parameterizations to study the effectiveness of the method. 
An initial observation, based on the data presented in the previous analysis and in \tableautorefname~\ref{tab:bd_variat} is that the optimal number of buckets is two.
In Section~\ref{sec:results}, we discuss the  the effectiveness of  the \gls{ba} algorithm for the specific configurations analyzed.


\begin{table}[b]
    %\normalsize
    \centering
    \caption{\scriptsize Fraction of attack alerts over all alerts varying $B$ and $D$. We are accounting all alerts, not following the detection's criterion.}
    \label{tab:bd_variat}
    \vspace{-0.05in}
    \setlength\tabcolsep{3pt} % default value: 6pt
    \begin{tabular}{ccr|ccr|ccr|ccr}
    \toprule
    \textbf{B} & \textbf{D} & \textbf{\%} & 
    \textbf{B} & \textbf{D} & \textbf{\%} & 
    \textbf{B} & \textbf{D} & \textbf{\%} & 
    \textbf{B} & \textbf{D} & \textbf{\%} \\\midrule
    1 & 30 & 7,71\% & 2 &  9 & 97,40\% & 2 & 15 & 98,01\% & 2 & 21 & 97,62\% \\
    2 & 6 & 92,22\% & 2 & 12 & 97,74\% & 2 & 18 & 98,01\% & 3 & 10 & 0,00\% \\\bottomrule
    
    \end{tabular}
\end{table}


==> commentTools.tex <==
\usepackage{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{soul}
\usepackage{graphicx}

 \usepackage[hidelinks]{hyperref}
% \AfterPreamble{\hypersetup{
%   hidelinks
% }}


\definecolor{mauve}{rgb}{0.58,0,0.82}
\definecolor{armygreen}{rgb}{0.29, 0.33, 0.13}
\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}

\newboolean{showcomments}
\setboolean{showcomments}{true}% TODO set false to disappear

\ifthenelse{\boolean{showcomments}}
{\newcommand{\mynote}[3]{\fbox{\bfseries\sffamily\tiny#1}% no space
{\scriptsize$\blacktriangleright$\textsf{\color{#3}{#2}}$\blacktriangleleft$}}}
{\newcommand{\mynote}[3]{}}

\newcommand{\na}[1]{\mynote{NA}{#1}{red}}
\newcommand{\nuno}{\na}
\newcommand{\antunes}{\na}
\newcommand{\mv}[1]{\mynote{MV}{#1}{mauve}}
\newcommand{\charles}[1]{\mynote{CG}{#1}{armygreen}}
\newcommand{\cg}{\charles}
\newcommand{\avz}[1]{\mynote{AA}{#1}{blue!50}}
\newcommand{\alberto}{\avz}
\newcommand{\beto}{\avz}
\newcommand{\daniel}[1]{\mynote{DM}{#1}{green}}

\newcommand{\toNA}[1]{\todo[inline, color=red!70]{\fbox{\bfseries\sffamily\scriptsize NA} #1}}
\newcommand{\toMV}[1]{\todo[inline, color=mauve!70]{\fbox{\bfseries\sffamily\scriptsize MV} #1}}
\newcommand{\toCG}[1]{\todo[inline, color=asparagus]{\fbox{\bfseries\sffamily\scriptsize CG} #1}}
\newcommand{\toAA}[1]{\todo[inline, color=blue!50]{\fbox{\bfseries\sffamily\scriptsize Alberto} #1}}
\newcommand{\toDM}[1]{\todo[inline, color=green]{\fbox{\bfseries\sffamily\scriptsize DM} #1}}


\newcommand{\wut}[0]{\fcolorbox{red}{white}{\bfseries\sffamily\tiny{\tiny$\blacktriangleleft$\textsf{\scriptsize\color{red}{(?)}}}}}
\newcommand{\MR}[0]{\fcolorbox{blue}{green}{\bfseries\sffamily\scriptsize{\small$\blacktriangleleft$\textsf{\color{blue}{REF}}}}}
%todo inline
\newcommand{\actionitem}[1]{\todo[inline]{\fbox{\bfseries\sffamily\scriptsize TODO} #1}}
%todo NOTE:
\newcommand{\note}[1]{\todo[inline, color=gray!10]{\fbox{\bfseries\sffamily\scriptsize Note} #1}}
%\newcommand{\note}[1]{\todo[inline, color=gray!10]{\fbox{\bfseries\sffamily\scriptsize Note} #1}}


==> oldabs.tex <==

%Virtualization enables Cloud Computing, allowing for server consolidation with cost reduction. It also introduces new challenges in terms of security and isolation, which are one of the roadblocks in their adoption in critical systems. Virtualized systems tend to be very complex, and multi-tenancy is the norm, as the hypervisor manages the resources shared amongst virtual machines. 
%This paper proposes a methodology that uses performance modeling for the detection of anomalies that can be triggered by dependability issues or security attacks in virtualized systems.
%The three-phase methodology profiles the system operation under normal conditions for every kind of transaction in every virtual host. The experimental results are used to calibrate a performance model. The calibrated model is used to validate the methodology parameters. Specifically, we evaluate the impact of bucket depth on the probability of false positives. Then, during the operation, the performance of the system is monitored, and deviations are detected using the bucket algorithm. 
%We demonstrate the methodology in a testing campaign using the TPCx-V workload, which was profiled during a set of executions. Then, we defined a set of resource exhaustion attacks to emulate the effects of anomalies affecting the performance of the system. The results show that our approach was able to successfully detect the anomalies, with a low number of false positives, and spot possibles residual effects on the system. 

% Virtualization enables Cloud Computing and allows for server consolidation with reduction of costs. 
% It also introduces new challenges in terms of security and isolation, which are one of the roadblocks in their adoption in critical systems. 
% Virtualized systems tend to be very complex, and multi-tenancy is the norm, as the hypervisor manages the resources shared amongst virtual machines. 
% This paper demonstrates the practical applicability of performance modeling approaches in the detection of anomalies that can be triggered, among other things,  by security attacks in virtualized systems. 
% For this, we designed a testing campaign based on the TPCx-V workload and a methodology on how to apply performance modeling to asses such a complex system.   First, we profiled the system operation under normal conditions for every kind of transactions in every virtual host. Then, we defined a set of resource exhaustion attacks to emulate anomalies that affect the performance of the system.  Finally, we used the bucket algorithm, tunned by the profile, to monitor the different transactions, and observed how many of those attacks the algorithm was able to report. 
% The results show that our approach was able to successfully detect the anomalies, with a low number of false positives, and spot possibles residual effects on the system.


==> transactionbased.tex <==
\subsection{ Benefits of Transaction-Based  Parametrization }

% \tableautorefname~\ref{tab:basel_alert_txns} shows  that 
 
Next, our goal is to reduce the number of false negatives reported in the previous section. To that aim, we  assess the benefits of % The  transactions  used in the benchmark have different  configurations. Therefore, we expect that allowing a
fine tuning  the anomaly detector, allowing a  distinct parametrization per transaction.  %, can produce  better performance results. %, sa different  for each operation.
% To that aim, %validate this intuition, % based on the data in \tableautorefname~\ref{tab:basel_alert_txns}, 
% we allowed the bucket depth  $D$ to vary between 6, 9, 12 and 15, associating one depth per transaction. % created a mix (Mix 6/9/12/15) for the , where the first  $D$ value for each transaction was used.  
 The performance results when $B=2$ and $D$ is allowed to vary between 12 and 15 are reported in %the upper part of 
 \tableautorefname~\ref{tab:cs2_tbl}.  % Allowing $D$ to vary only between 12 and 15 as in the previous section, the results are reported in the bottom part of  \tableautorefname~\ref{tab:cs2_tbl}. 
 \sadoc{how to choose between 12 and 15???}
 
 
 % \tableautorefname~\ref{tab:cs2_tbl} indicates that when restricting $D$ to vary in the range between 12 and 15 the performance sightly degrades in some cases (e.g., , but significantly improves improves in most scenarios.    
 
 
 \tableautorefname~\ref{tab:cs2_tbl} indicates that the fine tuning of the anomaly detector indeed reduces the number of false negatives when contrasted against results presented in the previous section (Table~\ref{tab:cs1_tbl}).  However, such gain comes at the cost of an increased number of false positives, as the reduction of the  bucket depth  favors premature alerts.  \emph{Given the model-based approach proposed in this paper, it is up to system designers to determine the desired cost function~\eqref{eq:cost1} so as to trade between detection time and false alarm rates.  Such tuning, in turn, can be executed in a system wide or in a per-transaction  basis, balancing between simplicity and  effectiveness.  }


\begin{table}[t]
    \tiny
    \centering
\caption{  Performance metrics for second case study \sadoc{keep only bottom part 12/15}}
    \label{tab:cs2_tbl}
    \includegraphics[width=0.9\linewidth]{./img/cs2_tbl.pdf}
\end{table}

% As a next tuning, following our analytical model, we avoided the values of $D$ below 12, by updating the values of 6 and 9 to 12. The results are shown in \tableautorefname~\ref{tab:cs2_tbl}.  We can conclude that there is opportunity for improved performance using adaptive tuning methods, specially for the {\it L} cases. 
%The exception is the {\it Ls} failure mode, that we already know that are not well covered by the method. 

% Therefore, for performance improvement, dynamic tuning methods~\cite{AvritzerBGTW06} could be used to balance the algorithm parameters. In addition, this observation reinforces the importance of applying  the methodology introduced in this paper.




